Probabilistically Correct Language-based Multi-Robot Planning using Conformal Prediction

This paper addresses task planning problems for language-instructed robot teams. Tasks are expressed in natural language (NL), requiring the robots to apply their capabilities at various locations and semantic objects. Several recent works have addressed similar planning problems by leveraging pre-trained Large Language Models (LLMs) to design effective multi-robot plans. However, these approaches lack performance guarantees. To address this challenge, we introduce a new distributed LLM-based planner, called S-ATLAS for Safe plAnning for Teams of Language-instructed AgentS, that is capable of achieving user-defined mission success rates. This is accomplished by leveraging conformal prediction (CP), a distribution-free uncertainty quantification tool in black-box models. CP allows the proposed multi-robot planner to reason about its inherent uncertainty in a distributed fashion, enabling robots to make individual decisions when they are sufficiently certain and seek help otherwise. We show, both theoretically and empirically, that the proposed planner can achieve user-specified task success rates, assuming successful plan execution, while minimizing the overall number of help requests. We provide comparative experiments against related works showing that our method is significantly more computational efficient and achieves lower help rates. The advantage of our algorithm over baselines becomes more pronounced with increasing robot team size.

==> experiment.tex <==
\section{Experiments}\label{sec:experiments}

In this section, we provide extensive comparative experiments to demonstrate the performance of our method. In Section \ref{sec:withbaseline}, we compare the proposed method against two commonly used multi-robot planning frameworks, centralized and decentralized methods. These experiments show that the performance gap between baselines and our method increases as the task complexity and the number of robots increase. In Section \ref{sec:cpresult}, we provide results in conformal prediction validation. In all case studies, we pick GPT-3.5\cite{brown2020language} as the LLM.

\subsection{Comparisons against LLM planners with traditional communication frameworks}\label{sec:withbaseline}

 \begin{table}[t]
 \centering
 \begin{tabular}{|c|c|}
 \hline
 Symbol & Explanation                      \\ \hline
 (1, X) & Locate and Go to the location of object/container X\\ \hline
 (2, X) & Pick up object X                 \\ \hline
 (3, X)    & Put down object at location X  \\ \hline
 (4, X) & Open the door of the container X \\ \hline
 (5)    & Let robot remain idle            \\ \hline
 \end{tabular}
 \caption{Action space used in Section \ref{sec:experiments}. The left column shows how each action in encoded in the prompt and the right one provides its explanation. $X$ is a variable referring to An object/region/container selected by the LLM. The plans $\tau$ are finite sequences of these actions.}
 \label{tab:symbol}
 \end{table}

\textbf{Setup:} We consider the following semantic objects $\ccalO= \{ \text{Apple, Kettle, Tomato, Bread, Potato, Knife, Coke} \}$ that can be recognized by the robot team. The environment is populated with two of the tomatoes, Coke, and kettle. Also there are one apple, one potato, one knife, and one loaf of bread. 
%
Meanwhile, there is a fridge where the status of its door is initialized to be closed. Hence as mentioned in the environment description in $\ell(t)$, a robot needs to open the door of the fridge before getting any item in it. Also here we assume that the locations of all objects as well as the fridge are accurate and the obstacle-free space is known. That means any robot in the team will know where to find the objects in the environment. The action space $\mathcal{A}$ is defined as in Table includes $5$ actions. % \textcolor{red}{[where is the set of actions?]}. 
%
The number of decisions that the LLM can pick from is $|\mathcal{S}|=28$. The action `let the robot remain idle' is useful when e.g., all the sub-tasks in $\phi$ have been assigned to other robots and the current robot can stay idle. Recall that the set is constructed using $\mathcal{A}$ and all objects/locations in the environment where actions in $\mathcal{A}$ can be applied. We select $T=60$ for all $\phi$ with a different number of sub-tasks. Notice that $T=H*N$, hence we consider multiple combinations of sub-tasks and robot numbers.


\begin{figure*}[!htp] 
\centering
\includegraphics[width=\linewidth]{img/single_robot_annotated.png} 
\caption{Case Study I: Execution of a single-robot plan for the mission: `Deliver a tomato and an apple to the sink. Also, deliver the kettle and the bread to the table'. Each snapshot illustrates a segment of the robot's plan to achieve each sub-task. } 
\label{fig:snapshot_single}
\end{figure*}

\textbf{Simulation Platform:} we demonstrate our method using AI2THOR platform\cite{kolve2017ai2, kannan2023smart}, on multi-robot mobile manipulation tasks using robots equipped with manipulator arms. A demonstration of the environment can be found in Figure \ref{fig:env}.

\textbf{Baseline:} In this work, we compare the performance of our method with two commonly used communication frameworks of multi-robot systems: decentralized\cite{mandi2023roco} and centralized\cite{chen2023scalable} methods. The decentralized method assigns an LLM agent for each robot in the team such that for every time step $t=\{1,\dots, H \}$, the LLM agent for robot $i\in \ccalI$ will generate the decision for its assigned robot with all the previous decision information. The centralized method assumes only one LLM agent such that for every time step $t$, LLM will generate plans for the entire team of $N$ robots simultaneously. Because we consider homogeneous robot teams, the hybrid framework proposed in \cite{chen2023scalable} which considers a central LLM planner that gives a global plan and the local LLM planner equipped by each robot justifies the feasibility of the plan, will be equivalent to a centralized method. Because any decision generated by LLM can be applied by all robots in the team so local LLM justification is not necessary. Notice that for the baselines, we provide LLMs with the given prompt but allow the models to predict/generate answers without converting all the action space into a multiple-choice-question-answering problem. We compare the accuracy of our method and two baselines over 110 case studies. For accuracy, we report the percentage of cases where a planner generates a plan that accomplishes the overall high-level task $\phi$ regardless of the number of sub-tasks. To make comparisons fair we have (i) exposed all three methods into the same set $\mathcal{S}$ and the prompt descriptions are the same; (ii) required for all the methods to have the same horizon $H$; (iii) removed all the CP elements in our method when we compare the performance with the baselines such that e.g., for robot $j$ at time $t$ are purely chosen based on $s_j(t)=\arg\max_{s\in\mathcal{S}}g(s|\ell_j(t))$
%
We classify the considered case studies into different categories based on the number of robots $N$ and sub-tasks $K$. Given that $T=H*N$, $H$ is fixed as $N$ is fixed, but $K$ can vary since we let LLMs reason and decide the assignment of the sub-tasks.


% \textcolor{red}{[are there any constraints in the task description? e.g., `robot $j$ should never touch the kettle'. I thought we had considered such cases. If so, mention that. Also, for each case, say something about the kind of mistakes that the LLM did. E.g., we had failures because it failed to open the fridge? It asked the robots to go to the wrong object? It did not generate a feasible sequence within $H$ steps? Are these mistakes the same across all case studies or you observed new mistakes as the number of robots increased?]}

% \textcolor{red}{[Here is my version for case study I. Provide the additional info I have included here in the other case studies too]}


% \textcolor{red}{[my draft]}
\textbf{Case Study I:} We consider $27$ scenarios with single-robot tasks (i.e., $N=1$) $\phi$ defined over four sub-tasks. Each sub-task requires moving a specific semantic object to a desired location $\bbx$. 
%
The safety constraint requires the robot to avoid approaching or grasping specific objects. For instance, a task may require the robot to move two tomatoes and one potato from the fridge to the kitchen counter  (three sub-tasks), put the bread in the microwave (one subtask). 
%
We select as maximum horizon $H=60$ for all scenarios considered in this case study.\footnote{Notice here we selected a large horizon because we constructed a single calibration dataset with single and multi robot tasks. A more efficient approach with respect to API calls, would be to have a separate calibration dataset for the single-robot case} The proposed planner designed correct plans in $27$ cases, i.e., the accuracy was $92.5\%$. 
%
The centralized and decentralized baseline achieved an accuracy of $37.2\%$; notice that when $N=1$ the two baselines trivially share the same planning scheme. We remark that although $H=60$, the robot manages to accomplish the task in a much shorter horizon $\bar{H}<H$; for $t>\bar{H}$, the action `do nothing' is selected. The average horizon $\bar{H}$ for our planner, centralized and decentralized baselines, across all successful scenarios, is 12, 13, and 13, respectively. Snapshots demonstrating a robot plan synthesized for one of the considered scenarios is shown in Figure \ref{fig:snapshot_single}.  % \textcolor{red}{[end of my draft]}


\begin{figure*}[!ht] 
\centering
\includegraphics[width=\linewidth]{img/3robot_annotated.png} 
\caption{Case Study II: Execution of a multi-robot plan for the mission: `Deliver the bread, apple and tomato to the table; Deliver the potato to the sink. Also, Robot 1 cannot pick up the knife'. The first 3 snapshots from left illustrate the plans generated for each robot to achieve the tasks, and the 4th snapshot shows the environment when all the tasks were finished. } 
\label{fig:snapshot_multi}
\end{figure*}

\textbf{Case Study II:} We consider 55 scenarios where the number of robots is $N=3$ with multi-robot tasks $\phi$ defined over either four or eight sub-tasks and at most one safety requirement. The safety usually applies to one of the robots in the team, e.g., robot $1$ cannot pick up the knife for safety reasons. 
%
The accuracy of the proposed method, centralized baseline, and decentralized baseline are $83.3\%$, $30.9\%$, and $27.3\%$, respectively. 
%
Here the average horizon $\bar{H}$ for our planner, centralized and decentralized baselines is $9$. 
%
Observe that the performance of our method remains comparable to the single-robot case. As we increase the number of robots $N$, failures occur in some of the scenarios using our method such as LLMs fail to respect the rule that the item inside the fridge cannot be directly accessed until the door is opened. Notice that here as the number of sub-tasks is larger than $N$, there will be at least one robot to be assigned with multiple sub-tasks. This lead to some of the scenarios that LLMs ask the robot to deliver the item to the wrong goal location when the robot is assigned with another sub-task after the first one is completed.
%
Snapshots demonstrating a robot plan synthesized for one of the considered scenarios is shown in Figure \ref{fig:snapshot_multi}.  

\textbf{Case Study III:} We consider 20 scenarios where the number of robots is $N=10$ with multi-robot tasks $\phi$ defined over either four or eight sub-tasks as well. Here we do not include the safety constraint due to the complexity caused by $N$. Notice here that the number of robots is larger than the number of sub-tasks, all the robots in the team will only be assigned to $0/1$ task in total. The accuracy of our planner, centralized baseline, and decentralized baseline are $95\%$, $60\%$, and $5\%$, respectively. The average horizon $\bar{H}$ for all three methods is $4$. Notice that even though the number of robots $N$ in this case is larger than the previous one, LLMs can still distinguish the requirements among the overall description and assign them to the robots accordingly. Observe that the accuracy of our method ($95\%$) is higher than case study II because here none of the robots will be assigned with multiple sub-tasks.


\textbf{Case Study IV:} Next, we consider 8 scenarios where the number of robots is $N=15$ with multi-robot tasks $\phi$ defined over ten sub-tasks. Here we do not include the safety constraint as well. In this case, all robots in the team will still be assigned to $0/1$ sub-task. The accuracy of our planner, centralized baseline, and decentralized baseline are $87.5\%$, $25\%$, and $0\%$, respectively. The average horizon $\bar{H}$ for all three methods is $4$. Here as the number of robots becomes much larger than in case study III, LLMs show a significant performance drop in the baseline methods as the models could not identify and categorize the useful information properly described in the prolonged prompt description and hence the performance especially in decentralized baseline becomes intractable. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[!t]
% \centering
% \begin{subfigure}[h]{0.49\linewidth}
% \includegraphics[width=\linewidth]{img/alpha85.png}
% \caption{$1-\alpha=0.85$}
% \label{fig:alpha85}
% \end{subfigure}
% \begin{subfigure}[h]{0.49\linewidth}
% \includegraphics[width=\linewidth]{img/alpha90.png}
% \caption{$1-\alpha=0.9$}
% \label{fig:alpha90}
% \end{subfigure}
% \caption{Empirical validation of conformal prediction sets. }
% \label{fig:cp_result}
% \end{figure}

% \subsection{Conformal Prediction Validation}\label{sec:cpresult}
% In this section, we empirically validate the mission success rates discussed in Section \ref{sec:theory}. We collect a calibration dataset $\ccalM$ with $M=50$ sequences. Then we collect a validation dataset collecting the scenarios discussed in Section \ref{sec:withbaseline} where if $\mathcal{C}(\bar{\ell}(k))$ is singleton, the assistance module described in Section \ref{sec:help} is activated to pick the decision. We conduct the following three experiments.

% In the first experiment,  we randomly sample $30$ calibration scenarios from our calibration set that will be used to construct prediction. Next, we randomly sample $50$ test scenarios and we compute the ratio of how many of the corresponding $50$ prediction sets contain the ground truth plan. We repeat 
% this $50$ times. When $1-\alpha=0.85$ and $1-\alpha=0.9$, the average ratio is $0.8588$ and $0.9072$, respectively, which are close to $0.85$ and $0.9$ as expected due to \eqref{eq:CP3} and Proposition \ref{prop:eq_prop}. 
% The histograms of these ratios are shown in Figure \ref{fig:cp_result}.

% In the second experiment, for each test sequence in our validation set, we sample a calibration set of $30$ sequences to construct prediction sets. Then, for each test scenario considered in Section \ref{sec:withbaseline}, we check if the constructed prediction set contains the correct plan. We compute the ratio of how many of the corresponding $110$ prediction sets contain the ground truth plan. We repeat  this $50$ times. When $1-\alpha=0.85$ and $1-\alpha=0.9$, the average ratio is $0.8596$ and $0.8942$, respectively, which are close to $0.85$ and $0.9$, as before, further validating the correctness of the constructed prediction sets. 

% Also, in the third experiment, we isolate the cases where singleton prediction sets $\bar{C}(\bar{\ell}_{\text{test}})$, defined in \eqref{eq:causalPred3},  were constructed. Among all these cases, when $1-\alpha=0.85$ and $1-\alpha=0.90$, in $91.26\%$ and $97.39\%$ of them, the correct plan was included in the prediction set. validating Theorem \ref{thm1}. 
% %
% When $1-\alpha=0.85$ and $1-\alpha=0.90$, the average percentage of local prediction sets $\ccalC(\ell_{\text{test}}(k))$ that were singletons was $98.89\%$ and $95.56\%$. This equivalently means that, e.g., when $1-\alpha=0.85$ on average, assistance was requested in making $1.11\%$ of all decisions $s_j(t)$. Observe that the frequency of asking for help increases as $1-\alpha$ increases, as expected. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Conformal Prediction Validation}\label{sec:cpresult}
In this section, we empirically validate the mission success rates discussed in Section \ref{sec:theory}. We collect a calibration dataset $\ccalM$ with $M=50$ sequences. Then we collect a validation dataset by considering the scenarios discussed in Section \ref{sec:withbaseline} where if $\mathcal{C}(\bar{\ell}(k))$ is singleton, the assistance module described in Section \ref{sec:help} is activated to pick the decision. We conduct the following experiment.

For each test sequence in the validation set, we sample a calibration set of $30$ sequences to construct prediction sets. Then, for each test scenario, we compute the robot plan using Alg. \ref{alg:MultiRobotLLM} with $W=0$ (to minimize API calls) and check if the robot plan is the ground truth plan. We compute the ratio of how many of the corresponding $110$ generated plans are the ground truth plan with respect to their corresponding tasks. We repeat this $50$ times. When $1-\alpha=0.85$ and $1-\alpha=0.90$, in $91.26\%$ and $97.39\%$ of them, the correct plan was equal to the generated robot plan. validating Theorem \ref{thm1}. 
%
%
When $1-\alpha=0.85$ and $1-\alpha=0.90$, the average percentage of local prediction sets $\ccalC(\ell_{\text{test}}(k))$ that were singletons was $98.89\%$ and $95.56\%$. This equivalently means that, e.g., when $1-\alpha=0.85$ on average, assistance was requested in making $1.11\%$ of all decisions $s_j(t)$. Observe that the frequency of asking for help increases as $1-\alpha$ increases, as expected. 



\subsection{Effect of the Ordered Set on the Prediction Set Size}
In this section, we demonstrate the effect of the ordered set $\ccalI$ on the prediction set size with 2 examples. Here the objects that can be recognized by the robots are one bottle of Coke, one apple, two tomatoes (denoted as T1, T2), and two loaf of bread (denoted as B1, B2).

First, we consider a scenario of $N=3$ where the task $\phi$ requires the robot team to deliver bread B2, apple to the table, deliver Coke to the stove and put the tomato to the sink. The initial ordered set is $\ccalI = \{1, 2, 3 \}$. In this scenario, the location of the bread B2 is inside the closed fridge that cannot be accessed directly by a robot until the door is opened. As we generate the prediction set at $t=1$ for the robot $\ccalI(1)=1$, a set of decisions \{(go to the location of bread B2), (go to the location of the fridge)\} is generated using CP. 
%
As mentioned in Section \ref{sec:help}, the help module is triggered when the prediction set has a size larger than $1$ by re-planning the time step $t$ using a new ordered set $\ccalI'$. Here we use $\ccalI' = \{2, 1, 3\}$. We observe for the new ordering $\ccalI'(1)=2$ (which means we are asking LLMs to generate decision for robot index $2$ instead of $1$ at $t=1$), the new prediction set now only includes a single action of \{(go to the location of the fridge)\} and hence the algorithm can proceed till completion without involving human in the loop. By the automated re-planning with a new ordered set $\ccalI'$, we reduce the chance of requesting help from human operators.

For another scenario of $N=3$ that requires robots to deliver bread B2 and tomato to the stove, put Coke to the desk, and put bread B1 to the table. With a task specifying different objects being delivered to different locations, LLMs show a similar performance as in the previous scenario that at $t=1$ when we use $\ccalI = \{1, 2, 3\}$, the prediction set for the robot $\ccalI(1)=1$ is \{(go to the location of bread B2), (go to the location of the fridge)\}. 
% 
As we trigger the help module, we re-plan time step $t=1$ using the new ordered set $\ccalI' = \{2, 1, 3\}$ and also observed that the prediction set reduce to singleton of going to the fridge location.

Note that as also discussed in Section \ref{sec:help}, using a new ordered set $\ccalI$ does not always lead to a smaller prediction set, in this section we picked 5 scenarios with non-singleton sets when $1-\alpha=0.9$, then we switch the ordered set and in 2 of them aforementioned, we managed to obtain a singleton prediction set in the corresponding time steps. 

% \subsection{Missions with Ambiguous Instructions}


% Here we demonstrate a case study when the instruction is ambiguous. Consider a task that requires a team of $N=3$ robots to deliver a tomato and a sweet drink to the table, and put the apple to the sink. In this case study, we have one apple, one tomato, one bottle of Sprite, and two bottles of Coke in the environment that could be recognized by the robot team. Firstly, two robots were assigned by LLM to finish the delivery of the tomato and the apple to their corresponding locations. When LLM generates the decision for the third robot, a prediction set of \{ (go to the location of Coke 1), (go to the location of Coke 2), (go to the location of Sprite) \} was generated by conformal prediction. Here notice that LLMs become uncertain about the task requirement given its common sense knowledge that 'both Coke and Sprite can be identified as sweet drinks'. To minimize the API calls, we use $W=0$ such that the human operator will choose the action (go to the location of Coke 2). 



==> intro.tex <==
\section{Introduction}

Multi-robot task planning is important in robotics due to its various applications such as housekeeping tasks\cite{benavidez2015design} and rescue missions\cite{queralta2020collaborative}. Yet planning for multi-robot systems is often challenging due to the coordination requirement during tasks as well as the complexity raised by the task horizon. Also, the difficulty increases drastically with the number of robots. Further, task sequencing and sub-task allocation are also crucial to the success of the overall task. Previous works have developed methods that are algorithm-based\cite{liu2023robust,cavorsi2023multi, chen2023autotamp} and learning-based\cite{zhang2022discovering}. They are usually tuned and fixed for a specific case which limits its generalization to new scenarios.

Motivated by the challenges in generalization to complex tasks and environments, Large Language Models(LLMs) have been broadly investigated in the field of robotics\cite{singh2023progprompt, liang2023code,shah2023lm,xie2023translating,ding2023task,liu2023llm+,wu2023tidybot,zeng2022socratic,stepputtis2020language,li2022pre,driess2023palm,huang2022inner,ruan2023tptu} to serve as the robot task planner, where it has shown its effectiveness in understanding complex task requirements described using Natural Language (NL). Besides, LLMs have also shown good logical reasoning and generalization abilities in different environments via prompt engineering techniques. As many of the works focus on single-agent systems, LLMs have also been explored recently within the multi-agent setup \cite{mandi2023roco, zhang2023building, kannan2023smart, chen2023scalable, rana2023sayplan, chen2024solving, yu2023co} where usually a separate LLM agent is assigned to each robot to engage in dialogue rounds for a potentially good plan. However, scalability becomes a great challenge in these works as the context information provided for each LLM contains related information for all other agents which makes the reasoning more difficult for language models and also might violate the token limitation of LLM APIs. Moreover, these works typically require a re-plan procedure whenever a local LLM discovers an error. Then the dialogue rounds will become intractable as the number of robots increases which increases the runtime of LLM inference and API costs. A more recent work\cite{chen2023scalable} proposed a hybrid planning framework that scales better as the number of robots increases, where they combine a global LLM planner with the local LLM agents. However, as NL has been explored as a more user-friendly means to specify robot missions; LLMs do not offer correctness guarantees to the generated answers. Several works have been proposed using conformal prediction to calculate such guarantees\cite{ren2023robots, wang2023conformal}. As these works focus on single-robot systems, it is non-trivial to scale them to multi-robot systems due to the number of LLM agents in the systems.

To mitigate the limitations mentioned above, we propose an alternative approach for multi-agent systems using LLMs that could be provided with satisfaction guarantees with conformal prediction while maintaining the scalability to larger robot teams and complex tasks. Our focus is on homogeneous robot teams tasked with performing high-level semantic sub-tasks (e.g., `deliver a bottle of water to the table') within the environment. We propose a new planner relying on a novel application of the coordinate descent method\cite{de2021random, ion2013rcd}, Large Language Models (LLMs)\cite{vaswani2017attention,devlin2018bert,raffel2020exploring,brown2020language,rae2021scaling,thoppilan2022lamda,wei2021finetuned, chowdhery2022palm}, and conformal prediction (CP)\cite{balasubramanian2014conformal,angelopoulos2023conformal,kumar2023conformal,ren2023robots,cleaveland2023conformal, wang2023conformal}. Specifically, first, we design a coordinate descent-based method using a robot index allocator such that plans at each step will be generated \textit{sequentially} for each robot based on the order created using the allocator. Then existing LLMs are employed to generate robot plans satisfying the given NL-specified tasks based on the given ordering. A key challenge here is that LLMs tend to hallucinate, i.e., to confidently generate outputs that are incorrect and possibly unrealistic \cite{lecun2023grounding}. This issue becomes more pronounced by potential ambiguity in NL-specified tasks. Thus, to reason about the correctness of the LLM-based plans, inspired by \cite{ren2023robots,kumar2023conformal,wang2023conformal}, we leverage CP \cite{angelopoulos2020uncertainty}. CP constructs on-the-fly prediction sets that contain the ground-truth/correct robot plan with a user-specified probability. This enables the robot to quantify confidence in its decisions and, therefore, comprehend \textit{when to seek for assistance} from human operators, to make mission progress. 

\textbf{Contribution:} The contribution of the paper can be summarized as follows. First, we propose a novel approach to design sequencing problems for multi-robot systems. Second, we provide a planning algorithm that relies on a novel integration of existing tools to design robot plans with probabilistic correctness guarantees for multi-robot systems. Fourth, we provide extensive comparative experiments demonstrating that the proposed planner outperforms related works.

==> method.tex <==
\section{Method}

In this section, we propose a new algorithm to address Problem \ref{pr:pr1}. In Section \ref{sec:coorddescent}, we provide a coordinate descent-based method such that each time the LLMs only consider the decision for a single robot in the team given all the previous information. In Section \ref{sec:llmplan}, we discuss how LLMs can be used to design plans $\tau$ satisfying the considered task and constraints. In Section  \ref{sec:cp}, using conformal prediction, we reason about the correctness of the plan with respect to the considered task. 

\begin{algorithm}[h]
\caption{Conformal Planning for Multi-Robot Systems with Large Language Models}\label{algo1}
\begin{algorithmic}[1]
\State \textbf{Input}: NL task description $\phi$; coverage guarantee $\alpha$; number of robots $N$;
\State Initialize robot index ordering $I_N=\{i_1, \dots, i_N\}$; 
\State Collect calibration set $\mathcal{M}$ and compute quantile $\bar{q}$
\State Construct initial prompt $\ell(0)$; decision set $\tau= \emptyset$; 
\For{$t=0~\text{to}~H-1$}
\For{$i\in I_N$}
\State Update index $i$ in prompt as $\ell_i(t)=\ell(t)+[i]$
\State Obtain scores $g(s|\ell_i(t)), \for s \in \mathcal{S}$
\State Compute $\mathcal{C}(\ell_i(t))=\{s | g(s|\ell_i(t)) > 1-\bar{q} \}$
\If{Prediction set $|\mathcal{C}(\ell_i(t))|>1$ }
\State Obtain help $s_i(t)$ from human operator
\Else
\State  Obtain  decision  $s_i(t)=\arg\max_s g(s|\ell_i(t))$
\EndIf
\State Update $\tau = \tau + [s_i(t)]$
\State Update prompt $\ell(t)=\ell_i(t)+[s_i(t)]$ 
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

\subsection{Coordinate Descent-Based Planning}\label{sec:coorddescent}

In this section, we present a coordinate descent-based planning scheme that generates plans for the robots in a pre-defined ordering. 

In traditional multi-robot planning methods, two communication frameworks are commonly employed within a robot team: decentralized and centralized. In the decentralized communication framework as described in \cite{mandi2023roco}, each robot is equipped with its own localized task planner, generating a single-step plan for its immediate task and subsequently communicating with the next robot in the team. However, this approach becomes less efficient as the number of robots and horizon increase and ultimately leads to a decline in performance, which limits its scalability. On the other hand, the centralized communication framework relies on a single global planner designing plans for all robots simultaneously at each step, but its performance degrades as the number of robots grows. In this work, we propose a novel planning approach that integrates the coordinate descent\cite{de2021random, ion2013rcd} method with a robot index allocator. This integration maintains planner performance even with an increasing number of robots and longer planning horizons, as we will discuss further and demonstrate its performance in subsequent sections.


\textbf{Robot Index Allocator:} For a team with $N$ robots, the allocator generates an ordering $I=[i_1, i_2, \dots, i_N]$ such that each element refers to a non-repeat index of a robot in the team. As we consider a homogeneous robot team in this work, the ordering will be equivalent to the ascending order of all robot indices in most of the cases, i.e., $I=[1, 2, \dots, N]$. 

\textbf{Coordinate Descent-based Method:} Different from the centralized communication framework where the planner generates actions for all robots in each step at once, we apply the concept of the coordinate descent method using a single planner for the entire robot team. At each time step $t\in \{0\dots H-1 \}$, the planner will make a decision only for a single robot at each query and iterate $N$ times sequentially following the order of the robots $I$ allocated above until all the robots in the team have been assigned to an action for the current time step.  In this process, the planner has access to all the decisions made thus far every time it generates a decision for the robot.

\begin{ex}[Feasible Plan Example(cont.)]
As we have a homogeneous team of $3$ robots, the ordering is initialized as the ascending order of robot indices $I=[1, 2, 3]$. As shown in $\tau$, at $t=0$, $s_1(\text{go to}, \text{Pen},1)$ refers to the decision for robot $1$ made by the planner is `go to the location of Pen'; $s_2(\text{go to}, \text{Coke},1)$ refers to the decision for robot $2$ is `go to the location of Coke' given that robot $1$ was assigned to finish the task related to Pen; robot $3$ is not assigned to any task and set to idle given all the previous assignments for both robot $1$ and $2$. Similarly, at $t=1$, the planner will generate decisions sequentially based on $I$ and all the decisions made in $t=0$.
\label{ex:me2} 
\end{ex}

\subsection{LLM Planner}\label{sec:llmplan}

Next, our goal is to design a plan $\tau$ based on the index allocation $I$ of robots. To synthesize $\tau$, we utilize existing LLMs as the planner. A key challenge is that LLMs cannot necessarily generate feasible instructions that are suitable for robot execution. For instance, an LLM response to the task `bring me a bottle of water' may be `go to the store and buy a bottle of water'.  This response is indeed reasonable but not executable due to the constraint of the environment. Therefore, we make LLMs be broken down into sequences of executable robot skills collected in $\ccalA$.

\textbf{Prompt Engineering:} To this end, we employ prompt engineering \cite{white2023prompt}.  Prompt engineering provides examples in the context text (`prompt') for the LLM  specifying the task and the response structure that the model will emulate. The prompt used in this work consists of the following parts \cite{wang2023conformal}.
\begin{enumerate}
    \item \textit{System description} that defines the action space determining all possible actions $s(a,\bbx,t)$ that all the robots can apply and rules that the LLM should always respect in its decision-making process. For instance, in our considered simulations, such rules explicitly determine that a robot cannot grasp an object located in a fridge before opening the fridge door. We observed that explicitly specifying such constraints improved the quality of LLM plans. We additionally require the length of the plan $\tau$ to be less than $H$, where $H\geq 0$ is a user-specified hyperparameter.
    \item \textit{Environment description} that describes the expected locations $\bbx_e$ of each semantic object $e$ of interest;
    \item  \textit{Task description} that includes the description of the task $\pi_{\text{next}}$ in natural language ; 
    \item \textit{History of actions} that includes the sequence of actions, generated by the LLM, that the robot team has been assigned so far towards accomplishing the assigned task;
    \item \textit{Response structure} describing the desired structure of the LLM output.
    \item \textit{Horizon and robot indicator} describing the current horizon step and which of the robots is the current planning target using the ordering $I$.
\end{enumerate}
% (1) \textit{System description} that defines the action space determining all possible actions $s(a,\bbx,t)$ that all the robots can apply and rules that the LLM should always respect in its decision-making process. For instance, in our considered simulations, such rules explicitly determine that a robot cannot grasp an object located in a fridge before opening the fridge door. We observed that explicitly specifying such constraints improved the quality of LLM plans. We additionally require the length of the plan $\tau$ to be less than $H$, where $H\geq 0$ is a user-specified hyperparameter.
% %
% (2) \textit{Environment description} that describes the expected locations $\bbx_e$ of each semantic object $e$ of interest;
% %
% (3) \textit{Task description} that includes the NL definition of the task $\pi_{\text{next}}$; 
% %
% (4) \textit{History of actions} that includes the sequence of actions, generated by the LLM, that the robot team has been assigned so far towards accomplishing the assigned task;
% %
% (5) \textit{Response structure} describing the desired structure of the LLM output.
% %
% (6) \textit{Horizon and robot indicator} describing the current horizon step and which of the robots is the current planning target using the ordering $I$.

\textbf{Plan Design:} In what follows, we describe how we use the above prompt to generate a plan $\tau$ incrementally so that our high-level task $\phi$ can be satisfied. The process of designing $\tau$ is converted into a sequence of $T>0$ multiple-choice question-answering problems for the LLM. Part $(4)$ and $(6)$ in the above prompt do not include any textual information initially at time $t=0$. We denote the prompt as $\ell(t)$ that include parts $(1)-(6)$ at time $t$. Given $\ell(t)$ and $I$, the LLM is asked to make a decision for robot $i\in I$ denoted as $s(a, \bbx, t)$ among all available ones included in part $(1)$. Notice that we consider homogeneous robot teams so the skills and their corresponding applications are the same among all robots. For simplicity, we adopt the notation $s(t)$ instead of $s(a, \bbx, t)$. We also denote by $\mathcal{S}$ all possible decisions $s$ that any robot can make; this set can be constructed offline using the action space $\ccalA$ and the available semantic objects. We obtain $N$ decision $s_i(t)$ for the robot with index $i$ in the team based on the ordering $I$ sequentially at each time step $t$ using the proposed planning scheme. 

We denote the initial prompt that includes parts $(1)-(6)$ at $t=0$ as $\ell(0)$.  Each time before we query the model with the prompt at time $t$, part $(6)$ will be updated with the robot index $i$ such that LLM is given explicit instruction that it's now the turn to plan for robot $i$ only. The prompt will be updated as 

\begin{equation}
\ell_i(t) = \ell(t) + [i]
\end{equation}
\noindent
where the summation means concatenation of text. Given any $s\in \mathcal{S}$, LLMs can provide a score $r(s|\ell_i(t))$; the higher the score, the more likely the decision $s$ is a valid next step to positively progress the task. Thus we query the model over all potential decisions $s$ and we convert them into a vector of `probabilities' using the softmax function \cite{wang2023conformal}. We denote the softmax score of the decision $s$ by $g(s|\ell_i(t))$. Then the decision for robot $i$ selected at time $t$ is denoted as:

\begin{equation}
s_i(t)=\arg\max_{s\in\mathcal{S}} g(s|\ell_i(t)).
\end{equation}

Notice here each time a decision is generated for a robot, we explicitly specify in the prompt the planning target $i$. We observe that LLMs tend to give a better performance with an explicit planning target. Once the $s_i(t)$ is selected for robot index $i$, we record $s_i(t)$ into part $(4)$. With slight abuse of notation, we denote the prompt update by

\begin{equation}
\ell(t) = \ell_i(t) + s_i(t)
\end{equation}
\noindent
where $\ell_i(t) + s_i(t)$ refers that the decision for robot index $i$ is recorded into the prompt. We repeat the above procedure for a total of $N$ times. Then we collect a set of decisions by iterating over all $N$ robots in the team at time $t$:

\begin{equation}
S(t) = \{s_i(t)\}, \forall i \in I
\end{equation}
\noindent
Once the set $S(t)$ containing all decisions for $N$ robots at time $t$ is collected, the robot team is deployed to execute the corresponding actions simultaneously as the current time step is updated to $t+1$.  Part $(4)$ and $(6)$ are being updated during the time interval $[0, H-1]$. This process generates a plan

\begin{equation}
\tau = S(0), S(1), \dots, S(H-1)
\end{equation}
\noindent
of horizon length $H$. The length of each $S(t)$ is $N$, and the plan $\tau$ is comprised of $T=H\times N$ decisions where each robot $i\in I$ will have its own decision set of $\{ s_i(0), s_i(1), \dots, s_i(H-1) \}$ corresponding to the set of decisions that this robot should follow. For a high-level task $\phi$ with $K\geq 1$ sub-tasks, we let LLMs reason about the current status of task assignment based on the prompt and generate decisions for each robot in the team.

\subsection{Probabilistic Satisfaction Guarantees for the Task}\label{sec:cp}

As discussed earlier, a key challenge lies in reasoning about the correctness of plan $\tau$. To address this challenge, inspired by \cite{ren2023robots, wang2023conformal, angelopoulos2021gentle}, we utilize an existing conformal prediction (CP) algorithm\cite{angelopoulos2020uncertainty}. CP allows us to provide probabilistic satisfaction guarantees for $\phi$. Specifically, we utilize CP to compute a prediction set that contains plans that satisfy the high-level task $\phi$ with high probability. Later, we show how to use this prediction set to reason about mission satisfaction. 

\textbf{Single-Robot-Single-Step Plans:} Here we focus on high-level task $\phi$ that can be satisfied by plans $\tau$ with a single decision such that $T=1$; this means synthesizing $\tau$ requires the LLM to make decision under the setup of $H=N=1$. Later we generalize the results for $T\geq 1$. 
%
First, we collect a calibration dataset $\ccalM=\{(\ell_{\text{calib}}^i,s_{\text{calib}}^i)\}_{i=1}^M$. 
%
We assume that there exists a unique correct decision $s_{\text{calib}}^i$ for each prompt $\ell_{\text{calib}}^i$. %This assumption can be relaxed exactly as in [CITE]. 
This assumption can be relaxed as in \cite{ren2023robots}; due to space limitations we abstain from this presentation.
%
Consider a new test data point $\ell_{\text{test}}$ %(denoted by $\ell(0)$ earlier) 
with unknown correct decision $s_{\text{test}}$. CP can generate a prediction set $\ccalC(\ell_{\text{test}})$ of decisions $s$ containing the correct one $s_{\text{test}}$ with probability greater than $1-\alpha$, i.e., 
%
%
\begin{equation}\label{eq:CP1}
P(s_{\text{test}}\in \mathcal{C}(\ell_{\text{test}})) \geq 1-\alpha,
\end{equation}
where $\alpha\in[0,1]$ is a user-specified coverage guarantee.
%
To generate $\mathcal{C}(\ell_{\text{test}})$, CP first uses the LLM’s confidence $g$ to compute the set of
nonconformity scores $\{r_i=1-g(s_{\text{calib}}^i~|~\ell_{\text{calib}}^i)\}_{i=1}^M$ over the calibration set.
%
The higher the score is, the less each data in the calibration set conforms to the data used for training the LLM. Then CP performs calibration by computing the $\frac{\ceil{(M+1)(1-\alpha)}}{M}$ empirical quantile of $r_1,\dots,r_M$ denoted by $q$. Then, it generates  prediction set 

\begin{equation}
\mathcal{C}(\ell_{\text{test}})=\{s\in \ccalS~|~g(s|\ell_{\text{test}})>1-q\}
\end{equation}
%
includes all labels (i.e., decisions) that the predictor is at least $1-q$ confident in. The generated prediction set ensures the $1-\alpha$ \textit{marginal} coverage guarantee, mentioned above, holds. By construction of the prediction sets, given a high-level task $\phi$, the LLM output plan $\tau=s(t)$ belongs to $\mathcal{C}(\ell_{\text{test}})$ meaning that the satisfaction probability of $\phi$ is greater than $1-\alpha$. A key assumption in CP is that all calibration and test data points are i.i.d. which holds in this setup. 

\begin{rem} [Dataset-Conditional Guarantee]\label{rem:datasetInd}
The probabilistic guarantee in \eqref{eq:CP1} is \textit{marginal} in the sense that the probability is over both the sampling of the calibration set $\ccalM$ and the test point $\ell_{\text{test}}$. Thus, a new calibration set will be needed for every single test data point $\ell_{\text{test}}$ to ensure the desired coverage guarantee $1-\alpha$, which is not practical. Thus, as introduced in \cite{vovk2012conditional}, we apply the following dataset-conditional guarantee which holds for a fixed calibration set across test data:
%
\begin{equation}\label{eq:data_cond_guarantee}
P(s_{\text{test}}\in \mathcal{C}(\ell_{\text{test}}) | \ccalM) \geq \text{Beta}^{-1}_{M+1-v, v}(\delta),
\end{equation}
\noindent
where $\text{Beta}^{-1}_{M+1-v, v}(\delta)$ denotes the quantile level of $\delta$ in a Beta distribution with $v= \left \lfloor{(M+1)\alpha_{\ccalM})}\right \rfloor$. 
%
Given a calibration dataset of size $M$ and a small value for $\delta$ ($\delta=0.01$), to achieve the desired coverage guarantee $1-\alpha$ (with probability $1-\delta$), we compute the parameter $\alpha_{\ccalM}$ so that
\begin{equation}
\alpha = 1- \text{Beta}^{-1}_{M+1-v, v}(\delta).
\end{equation}
\end{rem}

\textbf{Multi-Robot-Single-Step Plans:} We extend the above result to the case where the satisfaction of $\phi$ in the multi-robot-single-step setup that requires plans $\tau$ with $T \geq 1$ ($H=1, N\geq 1$) decisions selected from $\ccalS$. Here as we use the coordinate descent-based planning scheme, the test points are not independent of each other which violates the exchangeability assumption required by CP. The reason is that the prompts will be affected by the decisions made for all previous robots in the team. To address this challenge, as in \cite{ren2023robots}, the key idea is to (i) lift the data to sequences, and (ii) perform calibration at the sequence level using a carefully designed nonconformity score function.

First, we construct a calibration dataset as follows. We generate $M\geq1$ high-level tasks $\phi_i$. Each $\phi_i$ is broken into a sequence of $T=H*N\geq 1$ prompts with $N$ robots in the team and a horizon of $H=1$. Here the ordering of the robots is $I_N = \{j_1, \dots, j_N \}$ such that the sequence is denoted by:
%
\begin{equation}
\bar{\ell}_{\text{calib}}^i=[\ell_{\text{calib}}^{i,j_1}(0),\dots, \ell_{\text{calib}}^{i, j_N}(0)],
\end{equation}
%
Then for each prompt, we  manually construct the corresponding ground truth decisions denoted by
%
\begin{equation}
\tau_{\text{calib}}^i=s_{\text{calib}}^{i,j_1}(0),\dots,s_{\text{calib}}^{i,j_N}(0),
\end{equation}
%
Notice for the length of every $\bar{\ell}_{\text{calib}}^i$ and $\tau_{\text{calib}}^i$ is $N$.
%
This gives rise to the calibration set  $\ccalM=\{(\bar{\ell}_{\text{calib}}^i,\tau_{\text{calib}}^i)\}_{i=1}^M$.
%
Notice that based on the coordinate descent method, the prompts were built incrementally using the ordering of the robots $I_{N}$. 
%
As before, we assume that each context $\bar{\ell}_{\text{calib}}^i$ has a unique correct plan $\tau_{\text{calib}}^i$. Next, we use the lowest score over the entire sequence $j_1,\dots, j_N$ as the score  for each sequence in the calibration set, i.e., 
%
\begin{equation}
\bar{g}(\tau_{\text{calib}}^i~|~\bar{\ell}_\text{calib}^i)=\min_{j\in\{j_1,\dots, j_N\}}g(s_\text{calib}^{i,j}(0)~|~\ell_\text{calib}^{i,j}(0)),
\end{equation}
%
Thus, the non-conformity score of each sequence $i$ is
\begin{equation}\label{eq:non_conformity_score}
\bar{r}_i=1-\bar{g}(\tau_{\text{calib}}^i|\bar{\ell}_\text{calib}^i).
\end{equation}
%
Consider a new high-level task $\phi_{\text{test}}$ corresponding to a test data point $\bar{\ell}_{\text{test}}$ with unknown correct label/plan $\tau_{\text{test}}$ of length $T\geq 1$. CP can generate a prediction set $\bar{\ccalC}(\bar{\ell}_{\text{test}})$ of plans $\tau_{\phi}$ containing the correct one $\tau_{\text{test}}$  with high probability i.e., %{\phi,\text{test}}
\begin{equation}\label{eq:CP2}
P(\tau_{\text{test}}\in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}})) \geq 1-\alpha,
\end{equation}
where the prediction set $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is defined as 
%
\begin{equation}\label{eq:pred_set_2}
\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\{\tau~|~\bar{g}(\tau|\ell_{\text{test}})>1-\bar{q}\}, 
\end{equation}
%
where $\bar{q}$ is the $\frac{\ceil{(M+1)(1-\alpha)}}{M}$ 
%
empirical quantile of $\bar{r}_1,\dots,\bar{r}_M$. The generated prediction set ensures that the coverage guarantee in \eqref{eq:CP2} holds. By construction of the prediction sets, the plan $\tau_{\phi}$ generated by the LLM belongs to $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$.


\textbf{Causal Construction of the Prediction Set:} Observe that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is constructed after the entire sequence $\ell_{\text{test}}^{j_1}(0),\dots, \ell_{\text{test}}^{j_N}(0)$ is observed. 
%
However, at every step, the LLM observes only $\ell_{\text{test}}^{j}(0)$ and not the whole sequence. Thus, the prediction set needs to be constructed in a causal manner using only the current and past information. Thus, at every coordinate descent iteration $j$, we construct the causal prediction set  $\mathcal{C}(\ell^j_{\text{test}}(0)))=\{s~|~g(s|\ell^{j}_{\text{test}}(0)))>1-\bar{q}\}$. 
%
Then, the causal prediction set associated with $\bar{\ell}_{\text{test}}$ is defined as  $\mathcal{C}(\bar{\ell}_{\text{test}})=\mathcal{C}(\ell^{j_1}(0)))\times\mathcal{C}(\ell^{j_2}(0)))\dots\mathcal{C}(\ell^{j_N}(0)))$. As shown in \cite{ren2023robots}, $\mathcal{C}(\bar{\ell}_{\text{test}})$ and $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$, it holds that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}_{\text{test}})$.

\textbf{Multi-Robot-Multi-Step Plans:} Next, we generalize the above result to the case where the satisfaction of $\phi$ requires plans $\tau$ with $T \geq 1$ decisions selected from $\ccalS$. Here notice that $T\geq1$ refer to multi-robot-multi-step ($H\geq1, N\geq1$). Here the test points are also not independent of each other which violates the exchangeability assumption required to apply CP. 

In this case, we construct a calibration dataset as follows. We generate $M\geq1$ high-level tasks $\phi_i$, each consisting of $K_i$ sub-tasks in the NL description. Each $\phi_i$ is broken into a sequence of $T=H_i*N_i\geq 1$ prompts with $N_i\geq1$ robots in the team and horizon of $H_i\geq1$, denoted by:

\begin{equation}
\bar{\ell}_{\text{calib}}^i = 
[L_{\text{calib}}^i(0),\dots, L_{\text{calib}}^i(H_i-1)]
\end{equation}
\noindent 
where in this case each element $L_{\text{calib}}^i(t)$ is constructed sequentially using the robot index ordering $I_{N_i} = \{j_1, \dots, j_{N_i} \}$:
\begin{equation}
L_{\text{calib}}^i(t)=[\ell_{\text{calib}}^{i, j_1}(t),\dots, \ell_{\text{calib}}^{i, j_{N_i}}(t)],
\end{equation}
%
Then for each prompt, we  manually construct the corresponding ground truth decisions denoted by
%
\begin{equation}
\tau_{\text{calib}}^i=S_{\text{calib}}^i(0),\dots,S_{\text{calib}}^i(H_i-1),
\end{equation}
\noindent
where each element $S_{\text{calib}}^i(t)$ is written as 
\begin{equation}
S_{\text{calib}}^i(t)=s_{\text{calib}}^{i, j_1}(t),\dots,s_{\text{calib}}^{i, j_{N_i}}(t),
\end{equation}
%
This gives rise to the calibration set  $\ccalM=\{(\bar{\ell}_{\text{calib}}^i,\tau_{\text{calib}}^i)\}_{i=1}^M$.
%
Next, we use the lowest score over the entire sequence $0,\dots, T-1$ as the score for each sequence in the calibration set, i.e., 
%
\begin{equation}
\bar{g}(\tau_{\text{calib}}^i~|~\bar{\ell}_\text{calib}^i)=\min_{t\in\{0,\dots, H_i-1\}, j\in \{ j_1, \dots, j_{N_i}\}}g(s_\text{calib}^{i,j}(t)~|~\ell_\text{calib}^{i,j}(t)),
\end{equation}
%
Thus, the non-conformity score of each sequence $i$ can also be constructed as \eqref{eq:non_conformity_score}
\begin{equation}
\bar{r}_i=1-\bar{g}(\tau_{\text{calib}}^i|\bar{\ell}_\text{calib}^i).
\end{equation}
\noindent
Consider a new high-level task $\phi_{\text{test}}$ corresponding to a test data point $\bar{\ell}_{\text{test}}$ with unknown correct label/plan $\tau_{\text{test}}$ of length $T\geq 1$. We can also construct the prediction set as in \eqref{eq:pred_set_2} such that the coverage guarantee as in \eqref{eq:CP2} holds.
%
For a test data sequence $\bar{\ell}_{\text{test}}$, the prediction set is also constructed causally as  $\mathcal{C}(\bar{\ell}_{\text{test}})=\mathcal{C}(\ell^{j_1}(0)))\times\dots\times\mathcal{C}(\ell^{j_{N_{\text{test}}}}(0)))\times\dots\times\mathcal{C}(\ell^{j_1}(H_{\text{test}}-1)))\times\dots\times\mathcal{C}(\ell^{j_{N_{\text{test}}}}(H_{\text{test}}-1)))$ as proved above that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}_{\text{test}})$. Notice that $T = H_{\text{test}} * N_{\text{test}}$.
 
\textbf{Probabilistic LTL Satisfaction Guarantees:} Using the above CP framework, we can state the following result. 

\begin{theorem}\label{thm1}
With probability $1-\delta$ over the sampling of the calibration set $\ccalM$, the completion rate over new (but i.i.d.) test scenarios $\phi_{\text{test}}$ is at least $1-\alpha$, if $|\mathcal{C}(\ell_{\text{test}}^j(t)))|=1$, for all $t\in\{0,\dots,H_{\text{test}}-1\}$ and $j\in\{j_1, \dots, j_{N_{\text{test}}} \}$ i.e.,
$\mathbb{P}(\tau_{{\text{test}}}\models\phi_{\text{test}})\geq 1-\alpha$.
\end{theorem}

\begin{proof}
%\textcolor{red}{
This result follows directly from \eqref{eq:CP2}.
If $|\mathcal{C}(\ell^j_{\text{test}}(t)))|=1$, for all $t\in\{0,\dots,H_{\text{test}}-1\}$ and $j\in\{j_1, \dots, j_{N_{\text{test}}} \}$, then, since  $\mathcal{C}(\bar{\ell}_{\text{test}})=\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$, we have that \eqref{eq:CP2} is equivalent to $\mathbb{P}(\tau_{{\text{test}}}\models\phi_{\text{test}})\geq 1-\alpha$ (with probability $1-\delta$ as discussed in Remark \ref{rem:datasetInd}), completing the proof.
\end{proof}

\subsection{Seek for Assistance}

In this work, we assume whenever $|\mathcal{C}(\ell^j_{\text{test}}(t)))|>1$, for any $t\in\{0,\dots,H_{\text{test}}-1\}$ or $j\in\{j_1, \dots, j_{N_{\text{test}}} \}$, robot asks for help from human operator in order to proceed\cite{wang2023conformal,ren2023robots}. Specifically, the human operator will select the correct decision $s_j(t)$ for robot index $j$ at time step $t$.

==> method_new.tex <==
\section{Safe Planning for Language-Instructed Robot Teams}\label{sec:planner}

In this section, we propose a new decentralized mission planning algorithm that harness pre-trained LLMs to address Problem \ref{pr:pr1}. Specifically, in Section
\ref{sec:centralized}, we briefly present a centralized solution building upon \cite{ren2023robots}, which we show to be token inefficient. Motivated by this limitation, in Sections \ref{sec:centralized}-\ref{sec:help}, we proposed a decentralized planning framework. Specifically, in Section \ref{sec:coorddescent}, we show the task planning problem can be formulated as a sequence of multiple-choice question-answering (MCQA) scenarios. Then, in Section \ref{sec:cp} we show how this MCQA framework combined with conformal prediction (CP) can be combined to design planners with desired task success rates. When the latter is not possible, the robots seek assistance from each other or human operators as shown in Section \ref{sec:help}. In Section \ref{sec:theory}, we summarize the theoretical performance guarantees of the proposed framework.
%\ref{sec:coorddescent}, we provide a decentralized planning method that leverages recent advances in Large Language Models (LLM) to design robot plans. In Section \ref{sec:cp}, we reason about the correctness of the designed plan with respect to the considered task using conformal prediction (CP). As in \cite{ren2023robots,wang2023conformal}, we also discuss how CP enables individual robots to ask on-the-fly for help from human operators when they are uncertain about correctness of their actions. 
The proposed algorithm is summarized in Alg. \ref{alg:MultiRobotLLM}. 

% \textcolor{red}{[add refs to the algo lines throughout the text.]}


\subsection{A Centralized Planning Framework using LLMs}\label{sec:centralized}

%Existing (centralized or decentralized) multi-robot LLM-based planners to address Problem \ref{pr:pr1} often generate physically infeasible actions due to hallucinations of LLMs; see Section \ref{sec:intro}. This can be addressed by converting the mission planning problem into a multiple-choice question-answering (MCQA) problem as in \cite{ren2023robots,wang2023conformal,kumar2023conformal,ahn2022can}.
A potential solution to address Problem \ref{pr:pr1} is to directly apply the framework presented in \cite{ren2023robots} that is developed for single-robot task planning problems. The work in \cite{ren2023robots}, building upon \cite{ahn2022can,kumar2023conformal}, presents the task planning problem as a sequence of MCQA scenarios over time steps $t\in\{1,\dots,H\}$. In this setting, the question refers to the task $\phi$ along with a textual description of any possible mission progress. The choices refer to decisions $s_j(t)\in\ccalS$ that the (single) robot $j$ can make. Then, to pick the `best' action at time $t$, the LLM is queried $S=|\ccalS|$ times. A more detailed description can be found in \cite{ren2023robots}. This setting can be applied in the considered multi-robot planning problem by simply treating the multi-robot system as a single robot that can apply $N$ actions simultaneously. In this case, the number of choices/decisions $\bbs(t)$ in the MCQA framework are $S^N$. Thus, the employed LLM has to be queried $S^N$ times to pick a multi-robot action at a single time step $t$ which is impractical due to its token inefficiency. In fact, this can prohibitively increase the total API cost of using LLMs, especially, for long horizons $H$ or large number $N$ of robots. Also, the larger the number of choices in the MCQA framework is, the worse the planning performance gets, as shown by our empirical analysis. 

%Our empirical studies have also shown that the planning performan 


%all possible multi-robot actions $\bbs(t)$ that can be applied at time $t$. This eliminates plans that the LLM considers unlikely and reduces the problem of next-step prediction to a single next-token prediction. This process can be repeated sequentially over time, for some given horizon $H>0$, to design a plan $\tau$. A challenge within this centralized approach is that the number of choices $\bbs(t)$ increases exponentially fast as the number of robots or objects/regions increases making the reasoning more difficult for the language models \cite{chen2023scalable}. 


\begin{algorithm}[t]
\caption{Conformal Planning for Multi-Robot Systems with Large Language Models}\label{alg:MultiRobotLLM}
\begin{algorithmic}[1]
\State \textbf{Input}: NL task $\phi$; coverage guarantee $\alpha$; number of robots $N$; robot skills $\ccalA$; semantic environment $\Omega$
\State Initialize robot index ordering $\ccalI=\{1, \dots, N\}$; \label{algo1:order_init}
\State Collect calibration set $\mathcal{M}$ and compute quantile $\bar{q}$ \label{algo1:cp}
\State Construct initial prompt $\ell_1(t)$; decision set $\tau= \emptyset$; \label{algo1:prompt_init}
\For{$t=1~\text{to}~H$}
\For{$j=1~\text{to}~N$}
% \State Update index $i$ in prompt as $\ell_j(t)=\ell(t)+[i]$
\State Obtain scores $g(s_j|\ell_j(t)), \for s_j \in \mathcal{S}$ \label{algo1:score}
\State Compute $\mathcal{C}(\ell_j(t))=\{s_j | g(s_j|\ell_j(t)) > 1-\bar{q} \}$ \label{algo1:pred_set}
\If{Prediction set $|\mathcal{C}(\ell_j(t))|>1$ }
\State Obtain help $s_j(t)$ from human operator \label{algo1:help}
\Else
\State  Obtain  decision  $s_j(t)=\arg\max_{s_j} g(s_j|\ell_j(t))$
\EndIf
\State Update $\tau = \tau + [s_j(t)]$
\State Update $\ell_{j+1}(t)=\ell_j(t)+s_j(t)+``\text{robot }j+1"$ \label{algo1:prompt_update}
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}% \vspace{-0.5cm}
%\vspace{-3cm}
\normalsize

\subsection{Decentralized Multi-Robot Planning using LLMs}\label{sec:coorddescent}
%Our goal in this section is to design a planning algorithm capable of generating multi-robot mission plans $\tau$ accomplishing NL-expressed tasks $\phi$. We propose a coordinate descent-based planning algorithm that utilizes existing pre-trained LLMs to synthesize plans in a decentralized fashion. 
In this section, we propose a decentralized planning framework to address Problem \ref{pr:pr1} that is more token efficient than the one presented in Section \ref{sec:centralized}; see Remark \ref{rem:API}. Our setup leverages coordinate-descent methods that have been used extensively to address multi-robot planning problems in a decentralized manner \cite{atanasov2015decentralized,singh2009efficient}.
%allow the robots sequentially, as per some fixed order,  to design actions in a coordinate-descent manner. 
The key idea is that robots pick decisions at time $t$ successively (as opposed to jointly in Section \ref{sec:centralized}) using the MCQA setup, while incorporating the decisions of previous robots. In what follows, we describe our proposed decentralized planning algorithm in more detail.

%setting facilitating task reasoning and also significantly decreases the cost of using pre-trained LLMs. 



Consider a user-specified ordered set $\ccalI$ collecting the robot indices $j\in\{1,\dots,N\}$ where each robot index appears exactly once; e.g., $\ccalI=\{1,\dots,N\}$ [line \ref{algo1:order_init}, Alg. \ref{alg:MultiRobotLLM}]. We denote the $i-$th element in $\ccalI$ by $\ccalI(i)$. At each $t\in \{1\dots H \}$, the LLM will pick actions for each robot sequentially as per $\ccalI$. Specifically, robot $j=\ccalI(i)$ will select $s_j(t)$ while considering, all decisions that have been made until $t-1$, and all decisions made by the robots $\ccalI(1),\dots,\ccalI(i-1)$ at time $t$. Hereafter, for simplicity of notation, we assume that $\ccalI=\{1,\dots,N\}$ so that $\ccalI(j)=j$. %We note that such coordinate descent methods have been used to address various multi-robot planning problems in a more computationally efficient manner \cite{atanasov2015decentralized,singh2009efficient}.

%\begin{ex}[Feasible Plan Example(cont.)]
%As we have a homogeneous team of $3$ robots, the ordering is initialized as the ascending order of robot indices $I=[1, 2, 3]$. As shown in $\tau$, at $t=1$, $s_1(\text{go to}, \text{Pen},1)$ refers to the decision for robot $1$ made by the planner is `go to the location of Pen'; $s_2(\text{go to}, \text{Coke},1)$ refers to the decision for robot $2$ is `go to the location of Coke' given that robot $1$ was assigned to finish the task related to Pen; robot $3$ is not assigned to any task and set to idle given all the previous assignments for both robot $1$ and $2$. Similarly, at $t=2$, the planner will generate decisions sequentially based on $\ccalI$ and all the decisions made in $t=1$.
%\label{ex:me2} 
%\end{ex}

\textbf{Prompt Engineering:} In what follows, we discuss how each robot locally queries a pre-trained LLM to pick an action $s_j(t)$. The prompt used in this work consists of the following parts [line \ref{algo1:prompt_init}, Alg. \ref{alg:MultiRobotLLM}]. (1) \textit{System description} that defines the action space determining all possible actions $s_j(a,\bbx,t)$ that the robot can apply and rules that the LLM should always respect in its decision-making process. For instance, in our considered simulations, such rules explicitly determine that a robot cannot grasp an object located in a fridge before opening the fridge door. We observed that explicitly specifying such constraints improved the quality of LLM plans. We additionally require the length of the plan $\tau$ (i.e., the mission horizon) to be less than $H$, where $H\geq 0$ is a user-specified hyperparameter.
%
(2) \textit{Environment description} that describes the expected locations $\bbx_e$ of each semantic object $e$ of interest;
%
(3) \textit{Task description} that includes the task description $\phi$; 
%
(4) \textit{History of actions} that includes the sequence of actions, generated by the LLM, for all robots up to time $t-1$ and for all robots $1,\dots,j-1$ up to time $t$.
%
(5) \textit{Response structure} describing the desired structure of the LLM output for an example task.
%
(6) \textit{Current time step and robot index} describing the current time step $t$ and the index $j$ to the robot that is now responsible for picking an action as per $\ccalI$.

\textbf{Plan Design \& Execution:} Next, we describe how we use the above prompt to generate a feasible multi-robot plan $\tau$ incrementally. %so that our high-level task $\phi$ can be satisfied. 
The process of designing $\tau$ is converted into a sequence of $T>0$ MCQA scenarios for the LLM. Part $(4)$ in the above prompt does not include any textual information at time $t=0$. We denote the prompt associated with robot $j\in \ccalI$ at time $t$ by $\ell_j(t)$. %Also, we denote by $h(t, j)$ only part $(4)$ and $(6)$ of $\ell(t,j)$. 
Given $\ell_j(t)$ and $\ccalI$, the LLM is asked to select a decision $s_j(t)$, for robot $j$, among all available ones included in part (1). Given any $s_j(t)\in \mathcal{S}$, LLMs can provide a score $r(s_j(t)|\ell(t))$; the higher the score, the more likely the decision $s_j(t)$ is a valid next step to positively progress the task. To get the scores $r(s_j(t)|\ell(t))$ for all $s_j(t)\in \mathcal{S}$, we query the model over all potential decisions $s_j$ (i.e., $S=|\ccalS|$ times in total). Then, we convert them into a vector of normalized scores using the softmax function. We denote the softmax score of a decision $s_j$ by $g(s_j|\ell_j(t))$. 

Using these softmax scores, a possible approach to select the $s_j$ is by simply choosing the decision with the highest softmax score, i.e., $s_j(t)=\arg\max_{s_j\in\mathcal{S}} g(s_j|\ell_j(t))
$, as e.g., in \cite{ahn2022can}. However, this point-prediction approach is uncertainty-agnostic; note that these softmax scores do not represent calibrated confidence \cite{ren2023robots}. A much preferred approach would be to generate set predictions, denoted by $\ccalC(\ell_j(t))$ that contain the ground truth action with a user-specified high-probability. Hereafter, we assume that such prediction sets are provided; we defer their construction, using CP, to Section \ref{sec:cp} (see \eqref{eq:pred3local}). Given $\ccalC(\ell_j(t))$, we select decisions $s_j(t)$ based on the following two cases. If $\ccalC(\ell_j(t))$ is singleton, then we select the action included in $\ccalC(\ell_j(t))$ as it contributes to mission progress with high probability.\footnote{By construction of the prediction sets, this action coincides with $s_j(t)=\arg\max_{s_j\in\mathcal{S}} g(s_j|\ell_j(t))$; see Section \ref{sec:cp}}. Otherwise, robot $j$ seeks assistance from its teammates and/or a human operator to select $s_j(t)$. The latter is discussed in Section \ref{sec:help}.

%\begin{equation}
%s_j(t)=\arg\max_{s_j\in\mathcal{S}} g(s_j|\ell_j(t)).
%\end{equation}


Once $s_j(t)$ is selected, we record $s_j(t)$ into part $(4)$ and also update part $(6)$ by putting the next robot index $j+1$ based on the ordering $\ccalI$ into the prompt. With slight abuse of notation, we denote the prompt update by $\ell_{j+1}(t) = \ell_{j}(t) + s_j(t) + \text{`robot~$j+1$'},$ where the summation means concatenation of text [line \ref{algo1:prompt_update}, Alg. \ref{alg:MultiRobotLLM}]. We repeat the above procedure sequentially over all robots $j$ as per $\ccalI$. This way, we construct the multi-robot action $\bbs(t)$.
% here add the multi-robot setup 
Once $\bbs(t)$ is constructed, the robots execute their corresponding actions simultaneously, and the current time step is updated to $t+1$ in part (6).  Part (4) and (6) are being updated during the time interval $[t+1, t+H-1]$. This process generates the plan $\tau=\bbs(1),\dots,\bbs(t),\dots,\bbs(H)$ of horizon $H$. 
%Here as the length of each $S(t)$ is $N$, the plan $\tau$ is comprised of $T=H\times N$ decisions where each robot $i\in I$ will have its own decision set of $\{ s_i(0), s_i(1), \dots, s_i(H-1) \}$ corresponding to the trajectory this robot should follow. For a high-level task $\phi$ with $K\geq 1$ sub-tasks, we let LLMs reason about the current status of task assignment based on the prompt and generate decisions for each robot in the team.



\begin{rem}[Unknown \& Dynamic Environments]
    Recall from Section \ref{sec:problem} that we consider  environments where the locations of the semantic objects are known and fixed over time. To account for dynamic environments, at every time step $t$, once the multi-robot action $\bbs(t)$ is computed and executed, part (2) in the prompt should be updated to account e.g., for new or any missing objects.
\end{rem}

\begin{rem}[Token Efficiency Benefits]\label{rem:API}
    Observe that the number of choices/decisions $s_j(t)$ in the MCQA framework is $S$. Thus, to design the multi-robot action $\bbs(t)$, the LLM is queried $N\cdot S$ times, which is significantly smaller than $S^N$ required in the centralized approach in discussed Section \ref{sec:centralized}. This allows us to design multi-robot plans in a more token-efficient way, and mitigate the API costs incurred in the centralized setting which increase exponentially as the number of robots increases.
\end{rem}

\subsection{Decentralized Uncertainty Quantification using CP}\label{sec:cp}

In this section, we discuss how the prediction sets $\ccalC(\ell_j(t))$, introduced in Section \ref{sec:coorddescent}, are constructed, given a required task success rate $(1-\alpha)$\% (see Problem \ref{pr:pr1}). %As it will be shown in Section \ref{sec:theory}, these prediction sets allow us to characterize the task success rate of the proposed planner.
%
%A key challenge lies in reasoning about the correctness of plan $\tau$ with respect to $\phi$. To address this challenge, 
In what follows, inspired by \cite{ren2023robots}, we employ conformal prediction (CP) to construct these prediction sets. %to compute a prediction set that contains plans that satisfy the high-level task $\phi$ with high probability. Later, we show how to use this prediction set to reason about mission satisfaction. 
To better illustrate the challenges of their construction, we consider the following cases (that build upon each other): (i) single-robot \& single-step plans; (ii) multi-robot \& single-step plans; and (iii) multi-robot \& multi-step plans.

\textbf{Single-robot \& Single-step Plans:} Initially, we focus on cases where $N=1$ and on tasks $\phi$ that can be satisfied by plans $\tau$ with $H=1$. Later we generalize the results for $H\geq 1$ and $N\geq 1$. 
%
First, we collect a calibration dataset $\ccalM=\{(\ell_{j,\text{calib}}^i,\tau_{\text{calib}}^{i})\}_{i=1}^M$, using data drawn from $\ccalD$, where $\ell_{j,\text{calib}}^i$ is the prompt corresponding to the single robot $j$ for a task $\phi_i$ and $\tau_{\text{calib}}^{i}=s_{j,\text{calib}}^{i}(1)$ is the corresponding ground truth decision for robot $j$. Hereafter, we drop the dependence of the robot decisions on the time step, since we consider single-step plans. %Similarly, notice that we dropped the dependence of the prompt on the robot indices since we consider a single robot.
%
We assume that there exists a unique correct decision $s_{j,\text{calib}}^{i}$ for each $\ell_{j,\text{calib}}^i$. %This assumption can be relaxed exactly as in [CITE]. 
This assumption can be relaxed as in \cite{ren2023robots}; due to space limitations we abstain from this presentation.
%


Consider a new test data point $\ell_{j,\text{test}}$ (corresponding to a task $\phi_{\text{test}}$), drawn from $\ccalD$, %(denoted by $\ell(0)$ earlier) 
with unknown correct decision $s_{j,\text{test}}$ for robot $j$. CP can generate a prediction set $\ccalC(\ell_{\text{test}})$ of decisions $s_j$ containing the correct one $s_{j,\text{test}}$ with probability greater than $1-\alpha$, i.e., 
%
%
\begin{equation}\label{eq:CP1}
P(s_{j,\text{test}}\in \mathcal{C}(\ell_{j,\text{test}})) \geq 1-\alpha,
\end{equation}
where $\alpha\in[0,1]$ is user-specified.
%
To generate $\mathcal{C}(\ell_{j,\text{test}})$, CP first uses the LLM’s confidence $g$ to compute the set of
non-conformity scores (NCS) $\{r^i=1-g(s_{j,\text{calib}}^i~|~\ell_{j,\text{calib}}^i)\}_{i=1}^M$ over the calibration set.
%
The higher the score is, the less each data in the calibration set conforms to the data used for training the LLM. Then CP performs calibration by computing the $\frac{\ceil{(M+1)(1-\alpha)}}{M}$ empirical quantile of $r_1,\dots,r_M$ denoted by $q$. Then, it generates the prediction set 

\begin{equation}\label{eq:pred1}
\mathcal{C}(\ell_{\text{test}})=\{s_j\in \ccalS~|~g(s_j|\ell_{j,\text{test}})>1-q\},
\end{equation}
%
that includes all labels (i.e., decisions) that the predictor is at least $1-q$ confident in. This prediction set should be should be used to select decisions as per Section \ref{sec:coorddescent} for single-robot single-step tasks. 

The generated prediction set ensures that the $1-\alpha$ \textit{marginal} coverage guarantee, mentioned above, holds. By construction of the prediction sets the decision $s_j=\arg\max_{s_j\in\mathcal{S}} g(s_j|\ell_{j,\text{test}})$ belongs to $\mathcal{C}(\ell_{j,\text{test}})$. A key requirement in CP is that all calibration and test data points are i.i.d. which holds in this setup by assumption; see Problem \ref{pr:pr1}. 




\textbf{Multi-robot \& Single-step Plans:} Next, we generalize the above result to the multi-robot case, i.e., $N\geq 1$ while still considering tasks $\phi$ that can be satisfied by plans $\tau$ with horizon $H=1$. Notice that here we cannot apply directly \eqref{eq:CP1}-\eqref{eq:pred1} to compute individual prediction sets for each robot $j$ given a new task $\phi_{\text{test}}$. The reason is that the data points $\{(\ell_{j,\text{test}}(t),s_{j,\text{test}}(t))\}_{j=1}^N$ are not independent with each other which violates the exchangeability assumption required to apply CP. In fact, the distribution of prompts $\ell_{j,\text{test}}(t)$ depends on  decisions that have already been selected by the robots $1,\dots,j-1$ at time $t$. To address this challenge, the key idea is to (i) lift the data to sequences, and (ii) perform calibration at the sequence level using a carefully designed nonconformity score function. Hereafter, we drop the dependence on $t$, since we focus on single-step plans.

First, we construct a calibration dataset as follows. We generate $M\geq1$ high-level tasks $\phi_i$. %In what follows, we have that $t=1$ since $H=1$. 
Each $\phi_i$ is broken into a sequence of $N\geq 1$ prompts, where each prompt is structured as discussed in Section \ref{sec:coorddescent}. We define this sequence as:
%
\begin{equation}\label{eq:prompt2cal}
\bar{\ell}_{\text{calib}}^i=\ell_{1,\text{calib}}^i,\dots, \ell_{j,\text{calib}}^i,\dots,\ell_{N,\text{calib}}^i,
\end{equation}
where $\ell_{j,\text{calib}}^i$ is associated with robot $j$. %Notice that the order of robot indices $j$ in that sequence is determined by $\ccalI$. 
For each prompt, we  manually construct the corresponding ground truth decisions denoted by:
%
\begin{equation}\label{eq:plan2cal}
\tau_{\text{calib}}^i=\bbs_{\text{calib}}^i=[s_{1,\text{calib}}^i,\dots,s_{j,\text{calib}}^i,\dots, s_{N,\text{calib}}^i].
\end{equation}
%
This gives rise to the calibration set  $\ccalM=\{(\bar{\ell}_{\text{calib}}^i,\tau_{\text{calib}}^i)\}_{i=1}^M$.\footnote{Essentially, we assume that the calibration sequences \eqref{eq:prompt2cal}-\eqref{eq:plan2cal} are sampled from the (unknown) distribution $\ccalD$, introduced in Problem \ref{pr:pr1} \cite{ren2023robots}. Observe also that that these sequences share the same order of indices as per an ordered set $\ccalI_i$ (sampled from $\ccalD$ as part of $\phi_i$). Note that these ordered sets do not need not be the same across the calibration sequences. For simplicity of notation, in \eqref{eq:prompt2cal}-\eqref{eq:plan2cal}, we assume that that $\ccalI_i=\{1,\dots,N\}$ for all sequences $i$; we make the same assumption for the test sequence as well.} 
As before, we assume that each context $\bar{\ell}_{\text{calib}}^i$ has a unique correct plan $\tau_{\text{calib}}^i$. To apply CP, we need to associate each calibration point with a NCS. We define the NCS for each sequence $i$ in the calibration set as the lowest NCS over the individual decisions $s_{j,\text{calib}}^i(t)$ captured in $\tau_{\text{calib}}^i$ . Specifically, the score of the decisions $s_{j,\text{calib}}^i$ is $r_j^i=1-g(s_{j,\text{calib}}^i~|~\ell_{j,\text{calib}}^i)$, for all $j\in\{1,\dots,N\}$ (as defined in the single-robot \& single step plan case). Then, the NCS of the $i$-th calibration point is
\begin{equation}
\bar{r}_i=1-\bar{g}(\bbs_{\text{calib}}^i|\bar{\ell}_\text{calib}^i),
\end{equation}
%
where
\begin{equation}
\bar{g}(\bbs_{\text{calib}}^i~|~\bar{\ell}_\text{calib}^i)=\min_{j\in\{1,\dots, N\}}g(s_{j,\text{calib}}^i~|~\ell_{j,\text{calib}}^i).
\end{equation}

%
Consider a new high-level task $\phi_{\text{test}}$ corresponding to a prompt $\bar{\ell}_{\text{test}}={\ell}_{1,\text{test}},\dots,{\ell}_{j,\text{test}},\dots {\ell}_{N,\text{test}}$ with unknown correct label/plan $\tau_{\text{test}}$ of length $H=1$. CP can generate a prediction set $\bar{\ccalC}(\bar{\ell}_{\text{test}})$ of plans $\tau$ containing the correct one $\tau_{\text{test}}=\bbs_{\text{test}}(1)$  with high probability i.e., %{\phi,\text{test}}
\begin{equation}\label{eq:CP2}
P(\bbs_{\text{test}}\in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}})) \geq 1-\alpha,
\end{equation}
where the prediction set $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is defined as 
%
\begin{equation}\label{eq:pred2}
\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\{\bbs~|~\bar{g}(\bbs|\bar{\ell}_{\text{test}})>1-\bar{q}\}, 
\end{equation}
%
where $\bar{q}$ is the $\frac{(M+1)(1-\alpha)}{M}$ 
%
empirical quantile of $\bar{r}_1,\dots,\bar{r}_M$. The generated prediction set ensures that the coverage guarantee in \eqref{eq:CP2} holds. %By construction of the prediction sets, the single-step plan $\tau$ generated by the LLM belongs to $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$.

\underline{On-the-fly and Local Construction:}
Observe that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is constructed after the entire sequence $\bar{\ell}_{\text{test}}=\ell_{1,\text{test}},\dots,\ell_{N,\text{test}}$ is observed. This means uncertainty quantification of the LLM can be performed only after the whole plan is designed. %This may limit applicability of the proposed framework in offline missions.
%However, at every (test) time $t\in\{1,\dots,H_{\text{test}}\}$, the robot
%
%does not see the entire sequence $\bar{\ell}_{\text{test}}$ all at once; instead at every time $t\in\{1,\dots,H_{\text{test}}\}$
%observes only $\ell_{\text{test}}(t)$ and not the whole sequence. 
However, at test time, we do not see the entire sequence of prompts all at once; instead, the contexts $\bar{\ell}_{j,\text{test}}$ are revealed sequentially, one at a time. We thus need to construct the prediction set on-the-fly, using only the current and past information, as the robots take turns in querying the LLM for action selection.
%
Specifically, robot $j$ constructs the local prediction set 
\begin{equation}\label{eq:localPred2}
    %\centering
    \mathcal{C}(\ell_{j,\text{test}})=\{s_j~|~g(s_j|\ell_{j,\text{test}}))>1-\bar{q}\},
\end{equation}
where $g$ refers to the softmax score used in Section \ref{sec:coorddescent}. This set is a generalization of the prediction set in \eqref{eq:pred1} to multi-robot settings and should be used for decision making purposes in Section \ref{sec:coorddescent}. %Alternatively, %as in our implementation in Section \ref{sec:experiments},  
%$\mathcal{C}(\ell(t)))$ can be constructed using the RAPs approach that can result in smaller prediction sets \cite{angelopoulos2020uncertainty}; see Section \ref{sec:predSet}.
%
%
%Then, the causal prediction set associated with $\bar{\ell}_{\text{test}}$ is defined as  
%
% $\mathcal{C}(\bar{\ell}_{\text{test}})=\mathcal{C}(\ell(0)))\times\mathcal{C}(\ell(1)))\dots\mathcal{C}(\ell(H_{\text{test}})))$. 
%
As it will be shown in Section \ref{sec:theory}, it holds that 
\begin{equation}\label{eq:pred2c}%\mathcal{C}(\bar{\ell}_{\text{test}})
\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\ell_{1,\text{test}})\times\dots\times\mathcal{C}(\ell_{j,\text{test}})\times\dots\times\mathcal{C}(\ell_{N,\text{test}}).
\end{equation}
The result in \eqref{eq:pred2c} will be used in Section \ref{sec:theory} to provide task success rate guarantees for the proposed planner.
%
%As it will be shown shown in Section \ref{sec:theory}, it holds that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}_{\text{test}})$. 
%This causal construction of the prediction sets allow us to identify on-the-fly, i.e., as the multi-robot plan is constructed, for which robot $j$ and at what time step $t$, the LLM is uncertain about what the correct actions. This is particularly important for real-time missions where the robots $j$ should execute their decisions $s_j(t)$ as soon as they are made.






\textbf{Multi-robot \& Multi-step Plans:} Finally, we generalize the above result to the general case where $N\geq1$ and $H\geq 1$.
%multi-robot case (i.e., $N\geq 1$) where the accomplishing ta $\phi$ requires plans $\tau$ with $T > 1$ decisions selected from $\ccalS$. Here notice that $T>1$ may refer to a) single-robot-multi-step ($H>1, N=1$); b) multi-robot-single-step ($H=1, N>1$); or c) multi-robot-multi-step ($H>1, N>1$). 
%
Observe that we cannot apply \eqref{eq:localPred2} to compute  local prediction sets $\ccalC(\ell_{j,\text{test}}(t))$ associated with robot $j$ at every time step $t$.
%The challenge in this case is that the test points $\{(\ell_{\text{test}}(t+k,j),\bbs_{\text{test}}(t+k))\}_{k=1}^H$ are not independent with each other. 
%
The reason is that the distribution of prompts $\ell_{j,\text{test}}(t)$ depends on the previous prompts i.e., the multi-robot decisions at $t'<t$ as well as the decisions of robots $1,\dots,j-1$ at time $t$. To address this challenge, we will perform a similar analysis as in the previous case by performing calibration at the sequence level.

First, we construct a calibration dataset as follows [line \ref{algo1:cp}, Alg. \ref{alg:MultiRobotLLM}]. We generate $M\geq1$ high-level tasks $\phi_i$ defined over various number of robots $N_i$. Each task $\phi_i$ is broken into a sequence of $T=H_i\cdot N_i\geq 1$ prompts where $H_i$ is a task horizon associated with $\phi_i$.\footnote{As in the multi-robot \& single-step plan case,  we assume that the  sequences \eqref{eq:seqProm}-\eqref{eq:Plans3} are sampled from the (unknown) distribution $\ccalD$. This implies that the scenarios sampled from $\ccalD$ include also the number $N_i$ of robots as well as the ordered set $\ccalI_i$. As before, only for simplicity of notation, we assume ordered of the form $\{1,\dots,N\}$ for all calibration and test sequences.} This sequence of $T$ prompts is denoted by
%
\begin{align}\label{eq:seqProm}
&\bar{\ell}_{\text{calib}}^i=\underbrace{\ell_{1,\text{calib}}^i(1),\dots,\ell_{j,\text{calib}}^i(1),\dots,\ell_{N_i,\text{calib}}^i(1)}_{t=1},\dots,\nonumber\\&
%
\underbrace{\ell_{1,\text{calib}}^i(t'),\dots,\ell_{j,\text{calib}}^i(t'),\dots,\ell_{N_i,\text{calib}}^i(t')}_{t=t'},\dots,\nonumber\\&
%
\underbrace{\ell_{1,\text{calib}}^i(H_i),\dots,\ell_{j,\text{calib}}^i(H_i),\dots,\ell_{N_i,\text{calib}}^i(H_i)}_{t=H_i}.
\end{align}
%
Then, as before, for each prompt $\bar{\ell}_{\text{calib}}^i$, we  manually construct the corresponding sequence of ground truth decisions:
%
\begin{align}\label{eq:Plans3}
&\tau_{\text{calib}}^i=\underbrace{s_{1,\text{calib}}(1),\dots,s_{j,\text{calib}}(1),\dots,s_{N_i,\text{calib}}(1)}_{=\bbs(1)},\dots,\nonumber\\&
\underbrace{s_{1,\text{calib}}(t'),\dots,s_{j,\text{calib}}(t'),\dots,s_{N_i,\text{calib}}(t')}_{=\bbs(t')},\dots,\nonumber\\&
\underbrace{s_{1,\text{calib}}(H_i),\dots,s_{j,\text{calib}}(H_i),\dots,s_{N_i,\text{calib}}(H_i)}_{=\bbs(H_i)}.
\end{align}
%
\noindent
This gives rise to the calibration set  $\ccalM=\{(\bar{\ell}_{\text{calib}}^i,\tau_{\text{calib}}^i)\}_{i=1}^M$.
%
%Notice that the prompts were built sequentially as per the coordinate descent method. Hence with a horizon of $H_i$ for task $\phi_i$, the sequence of prompts $\bar{\ell}_{\text{calib}}^i$ can be  rewritten into the form of 
%\begin{equation}
%\bar{\ell}_{\text{calib}}^i = 
%[L_{\text{calib}}^i(0),\dots, L_{\text{calib}}^i(H_i-1)]
%\end{equation}
%\noindent 
%where $L_{\text{calib}}^i(t) = \{ \ell_{\text{calib}}^{i, j}(t) \}, \forall j\in I_{N_i}$ refers to the prompts for each robot $j$ at time step $t$.
%
%Also, ground truth decision sequence can be written as 
%\begin{equation}
%\tau_{\text{calib}}^i=S_{\text{calib}}^i(0),\dots,S_{\text{calib}}^i(H_i-1),
%\end{equation}
%\noindent
%where $S_{\text{calib}}^i(t) = \{ s_{\text{calib}}^{i, j}(t) \}, \forall j \in I_{N_i}$. Here each time step $t$ will include $N_i$ prompts and decisions corresponding to all robots in the team.
%
As before, we assume that each context $\bar{\ell}_{\text{calib}}^i$ has a unique correct plan $\tau_{\text{calib}}^i$.
%
Hereafter, we denote by $\bar{\ell}_{\text{calib}}^i(k)$ and $\tau_{\text{calib}}^i(k)$ the $k$-th entry in the sequences $\bar{\ell}_{\text{calib}}^i$ and $\tau_{\text{calib}}^i$, respectively, where $k\in\{1,\dots,T\}$. Note that $k$ is different from the time step $t\in\{1,\dots,H_i\}$ and that $T$ is the same across all calibration points. 

Next, for each calibration datapoint, we define the NCS similarly to the multi-robot-single-step plan case. Particularly, the score of a decision $\tau_{\text{calib}}^i(k)$ is $r_k^i=1-g(\tau_{\text{calib}}^i(k)~|~\ell_\text{calib}^i(k))$, for all $k\in\{1,\dots,T\}$. Then, the NCS of the multi-robot plan $\tau_{\text{calib}}^i$ is the lowest score over $k\in\{1,\dots,T\}$, i.e., 
%
\begin{equation}
\bar{g}(\tau_{\text{calib}}^i~|~\bar{\ell}_\text{calib}^i)=\min_{k\in\{1,\dots, T\}}g(s_\text{calib}^i(k)~|~\ell_\text{calib}^i(k)).
\end{equation}
%
Thus, the NCS of each calibration sequence $i$ is
\begin{equation}
\bar{r}_i=1-\bar{g}(\tau_{\text{calib}}^i|\bar{\ell}_\text{calib}^i).
\end{equation}

Consider a new task $\phi_{\text{test}}$, defined over $N_{\text{test}}$ robots, corresponding to a test data point $\bar{\ell}_{\text{test}}=\bar{\ell}_{\text{test}}(1),\dots,\bar{\ell}_{\text{test}}(k),\dots,\bar{\ell}_{\text{test}}(T)$ with unknown correct label/plan $\tau_{\text{test}}$. We select the mission horizon $H_\text{test}\geq 1$ so that $T=H_\text{test}\cdot N_{\text{test}}$.
%
Using CP, we can generate a prediction set $\bar{\ccalC}(\bar{\ell}_{\text{test}})$ of plans $\tau$ containing the correct one $\tau_{\text{test}}$  with high probability i.e., %{\phi,\text{test}}
\begin{equation}\label{eq:CP3}
P(\tau_{\text{test}}\in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}})) \geq 1-\alpha,
\end{equation}
where the prediction set $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is defined as [line \ref{algo1:pred_set}, Alg. \ref{alg:MultiRobotLLM}] 
%
\begin{equation}\label{eq:pred3}
\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\{\tau~|~\bar{g}(\tau|\ell_{\text{test}})>1-\bar{q}\}, 
\end{equation}
%
where $\bar{q}$ is the $\frac{(M+1)(1-\alpha)}{M}$ 
%
empirical quantile of $\bar{r}_1,\dots,\bar{r}_M$. The generated prediction set ensures that the coverage guarantee in \eqref{eq:CP3} holds. %By construction of the prediction sets, the plan $\tau$ generated by the LLM belongs to $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$. 
%
The size of the prediction sets can be used to evaluate uncertainty of the LLM. Specifically, if $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is singleton then this means that the LLM is certain with probability at least $1-\alpha$ that the designed multi-robot accomplishes the assigned task.
%

\underline{On-the-fly and Local Construction:}
Observe that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ in \eqref{eq:pred3} is constructed after the entire sequence $\bar{\ell}_{\text{test}}=\bar\ell_{\text{test}}(1),\dots,\bar\ell_{\text{test}}(T)$ is observed. %This means uncertainty quantification of the LLM can be performed only after the whole plan is designed. %This may limit applicability of the proposed framework in offline missions.
%However, at every (test) time $t\in\{1,\dots,H_{\text{test}}\}$, the robot
%
%does not see the entire sequence $\bar{\ell}_{\text{test}}$ all at once; instead at every time $t\in\{1,\dots,H_{\text{test}}\}$
%observes only $\ell_{\text{test}}(t)$ and not the whole sequence. 
Similarly to the previous case, next we discuss how the prediction set can be constructed on-the-fly.
%
At every iteration $k$, we construct the local prediction set associated with a robot $j$ and a time step $t$,  
\begin{equation}\label{eq:pred3local}
    \mathcal{C}(\bar{\ell}_{\text{test}}(k)))=\{\tau_{\text{test}}(k)~|~g(\tau_{\text{test}}(k)|\bar{\ell}_{\text{test}}(k)))>1-\bar{q}\},
\end{equation}
where $g$ refers to the softmax score used in Section \ref{sec:coorddescent}. This prediction set should be used to select robot decisions $s_j(t)$ as discussed in Section \ref{sec:coorddescent}. Also, notice that
%generalizes the prediction sets \eqref{eq:pred1} and \eqref{eq:localPred2} to multi-robot and multi-step plans. In other words, 
\eqref{eq:pred3local} degenerates to \eqref{eq:localPred2} if $H_{\text{test}}=1$ and $N_{\text{test}}>1$, and to \eqref{eq:pred1} if $H_{\text{test}}=1$ and $N_{\text{test}}=1$.
%
%Alternatively, %as in our implementation in Section \ref{sec:experiments},  
%$\mathcal{C}(\ell(t)))$ can be constructed using the RAPs approach that can result in smaller prediction sets \cite{angelopoulos2020uncertainty}; see Section \ref{sec:predSet}.
%
%
%Then, the causal prediction set associated with $\bar{\ell}_{\text{test}}$ is defined as  
%
% $\mathcal{C}(\bar{\ell}_{\text{test}})=\mathcal{C}(\ell(0)))\times\mathcal{C}(\ell(1)))\dots\mathcal{C}(\ell(H_{\text{test}})))$. 
%
%
%
As it will be shown shown in Section \ref{sec:theory}, it holds that 
\begin{equation}\label{eq:pred3c}
\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}(0)))\times\mathcal{C}(\bar{\ell}(1)))\dots\mathcal{C}(\bar{\ell}(k)))\dots\times\mathcal{C}(\bar{\ell}(T))).
\end{equation}
%$\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}_{\text{test}})$. 
Observe that \eqref{eq:pred3local}-\eqref{eq:pred3c} is a generalization of \eqref{eq:localPred2}-\eqref{eq:pred2c} for multi-step plans. This result is critical to showing that the proposed planner is supported by the task success rates discussed in Problem \ref{pr:pr1}. Finally,  this causal construction of the prediction sets allow us to identify on-the-fly, i.e., as the multi-robot plan is constructed, for which robot $j$ and at what time step $t$, the LLM is uncertain about the correct decisions. This is particularly important for real-time missions where the robots should execute their decisions $s_j(t)$ as soon as they are made.

\begin{rem}[Communication Architecture]

The approach for the construction of the prediction set 
$\bar{\ccalC}(\bar{\ell}_{\text{test}})$ in \eqref{eq:pred3c} is not fully-distributed because multi-hop
communication is needed to pass information across robots. However, all-to-all communication is not required either because the construction of the prediction sets and, consequently, the decision making process (Section \ref{sec:coorddescent}) naturally occurs in communication hops. 
%
To construct the prediction sets and select decisions $s_j(t)$, the robots should transmit to each other their current decisions in order to compute the history of actions required to construct part (4) in the prompt $\bar{\ell}_{\text{test}}$; see Section \ref{sec:coorddescent}.
%    
\end{rem}

\begin{rem} [Dataset-Conditional Guarantee]\label{rem:datasetInd}
The probabilistic guarantee in \eqref{eq:CP3} is \textit{marginal} in the sense that the probability is over both the sampling of the calibration set $\ccalM$ and the test point $\ell_{\text{test}}$. Thus, a new calibration set will be needed for every single test data point $\bar{\ell}_{\text{test}}$ to ensure the desired probability $1-\alpha$, which is not practical. Thus, as in \cite{vovk2012conditional}, we can apply the following dataset-conditional guarantee which holds for a fixed calibration set across test data:
%
\begin{equation}\label{eq:data_cond_guarantee}
P(\tau_{\text{test}}\in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}}) | \ccalM) \geq \text{Beta}^{-1}_{M+1-v, v}(\delta),
\end{equation}
\noindent
where $\text{Beta}^{-1}_{M+1-v, v}(\delta)$ denotes the quantile level of $\delta$ in a Beta distribution with $v= \left \lfloor{(M+1)\alpha_{\ccalM})}\right \rfloor$. 
%
Given a calibration dataset of size $M$ and a small value for $\delta$ ($\delta=0.01$), to achieve the desired coverage guarantee $1-\alpha$ (with probability $1-\delta$), we compute the parameter $\alpha_{\ccalM}$ so that $\alpha = 1- \text{Beta}^{-1}_{M+1-v, v}(\delta)$.
\end{rem}


\subsection{Seeking Assistance from Teammates and Human Operators}
\label{sec:help}

%\textbf{Ask-for-Help:} 
As discussed in Section \ref{sec:coorddescent}, if $\mathcal{C}(\ell(k)))$ is singleton, then this means that the LLM is certain that the decision $s_j(t)$ included in  $\mathcal{C}(\ell(k)))$ will contribute to making mission progress. Otherwise, the corresponding robot seeks assistance in two ways [line \ref{algo1:help}, Alg. \ref{alg:MultiRobotLLM}]. First, a message is sent to all previous robots asking them to re-plan their actions for the time step $t$ but in a different order $\ccalI$.
%we change the $\ccalI$ and ask the robots to re-plan their actions for the current time-steps, 
We iterate over various ordered sets $\ccalI$ until singleton prediction sets are generated for all robots.\footnote{Notice that this step may be computationally expensive to perform online and it may also increase the cost of using LLMs. Thus, it may be neglected for large robot teams and action spaces. \textcolor{red}{[we can delete the following, as it is kinda repetitive, once you confirm you agree with it]} Also, notice %that quantile $\bar{q}$ used to compute the prediction sets may depend on $\ccalI$; 
that given a fixed task $\phi$, different ordered 
order sets $\ccalI$ will yield different sequences of prompts in \eqref{eq:seqProm}. This may result in different NCS for calibration sequences, and, consequently, in a different quantile $\bar{q}$ (for a fixed $1-\alpha$). Thus, a test-time sequence of prompts $\bar{\ell}_{\text{test}}$ constructed using $\ccalI$ that is different from the one used in the construction of the calibration dataset may violate the i.i.d. assumption required to apply CP. This in turn may invalidate the provided coverage guarantees (although this is challenging to formally prove). This can be mitigated by considering calibration data points of various, instead of fixed, ordered sets $\ccalI$.
%
%
%changing the order in $\ccalI$ at test time does not violate the coverage guarantees discussed in Section \ref{sec:cp}, as long as the distribution $\ccalD$ can generate tasks (i.e., sequences of prompts $\bar{\ell}_{\text{test}}$ defined in Section \ref{sec:cp}) as per the new order $\ccalI$. Otherwise, changing the order in $\ccalI$ may violate the i.i.d. assumption required to apply CP (although this is challenging to formally prove).
} Our empirical analysis has shown that $\ccalI$ can affect the size of prediction sets; see \ref{sec:experiments}. 
If such a set $\ccalI$ cannot be found, the robots request  help from human operators as in \cite{ren2023robots}. Particularly, the robot presents to a user the set $\mathcal{C}(\ell(k)))$ (along with the prompt $\ell(k)$) and asks them to choose one action from it. The operator man either picks an action for the corresponding robot or decides to halt operation.

%\begin{rem}[CP \& Dynamic Order $\ccalI$]
%\textcolor{red}{[maybe we should remove this...]}
%We note here that changing the order of robot indices in  $\ccalI$ at test-time would violate the coverage guarantees provided in Section \ref{sec:cp} if the robots were heterogeneous in their skills. The reason is that this may switch the ground truth plans/labels in the calibration dataset from feasible to infeasible (which is not the case in the considered homogeneous robot case). Consequently, this would change the quantiles used to construct the prediction sets.  
%Notice that changing the order in $\ccalI$ at test time does not violate the coverage guarantees, as long as the distribution $\ccalD$ can generate tasks (i.e., sequence of prompts $\bar{\ell}_{\text{test}}$ defined in Section \ref{sec:cp}) as per the new order. Otherwise, changing the order in $\ccalI$ may violate the i.i.d. assumption required to apply CP.
%\end{rem}


\subsection{Theoretical Guarantees for Mission Success Rate}\label{sec:theory}
 
% \textcolor{red}{[put here two results. One about the causal prediction and one about the mission success rates. It's fine to say that the proofs are similar to the ones in princeton and that we present them here for completeness of the paper]}

\textbf{Causal Construction of Prediction Set:} Observe that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is constructed after the entire sequence $\bar{\ell}_{\text{test}}$ is observed. 
%
However, at every step $k\in \{1,\dots,T \}$, the LLM observes only $\bar{\ell}_{\text{test}}(k)$ and not the whole sequence. Thus, the prediction set needs to be constructed in a causal manner using only the current and past information. Thus, at every step $k$, we construct the causal prediction set  $\mathcal{C}(\bar{\ell}_{\text{test}}(k)))=\{s~|~g(s|\bar{\ell}_{\text{test}}(k)))>1-\bar{q}\}$. 
%
Then, the causal prediction set associated with $\bar{\ell}_{\text{test}}$ is defined as  $\mathcal{C}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}_{\text{test}}(1)))\times\mathcal{C}(\bar{\ell}_{\text{test}}(2)))\dots\mathcal{C}(\bar{\ell}_{\text{test}}(T)))$. As shown in \cite{ren2023robots}, $\mathcal{C}(\bar{\ell}_{\text{test}})$ and $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$, it holds that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}_{\text{test}})$.

\textbf{Probabilistic LTL Satisfaction Guarantees:} Using the above CP framework, we can state the following result. 

\begin{theorem}\label{thm1}
With probability $1-\delta$ over the sampling of the calibration set $\ccalM$, the completion rate over new (but i.i.d.) test scenarios $\phi_{\text{test}}$ is at least $1-\alpha$, if $|\mathcal{C}(\bar{\ell}_{\text{test}}(t)))|=1$, for all $t\in\{1,\dots,T\}$ i.e.,
$\mathbb{P}(\tau_{{\text{test}}}\models\phi_{\text{test}})\geq 1-\alpha$.
\end{theorem}

\begin{proof}
%\textcolor{red}{
This result follows directly from \eqref{eq:CP2}.
If $|\mathcal{C}(\bar{\ell}_{\text{test}}(t))|=1$, for all $t\in\{0,\dots,T\}$, then, since  $\mathcal{C}(\bar{\ell}_{\text{test}})=\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$, we have that \eqref{eq:CP2} is equivalent to $\mathbb{P}(\tau_{{\text{test}}}\models\phi_{\text{test}})\geq 1-\alpha$ (with probability $1-\delta$ as discussed in Remark \ref{rem:datasetInd}), completing the proof.
\end{proof}

==> method_new2.tex <==
\section{Safe Planning for Language-Instructed Robot Teams}\label{sec:planner}

In this section, we propose a new decentralized mission planning algorithm that harness pre-trained LLMs to address Problem \ref{pr:pr1}. Specifically, in Section
\ref{sec:centralized}, we briefly present a centralized solution building upon \cite{ren2023robots}, which we show to be token inefficient. Motivated by this limitation, in Sections \ref{sec:centralized}-\ref{sec:help}, we proposed a decentralized planning framework. Specifically, in Section \ref{sec:coorddescent}, we show the task planning problem can be formulated as a sequence of multiple-choice question-answering (MCQA) scenarios. Then, in Section \ref{sec:cp} we show how this MCQA framework combined with conformal prediction (CP) can be combined to design planners with desired task success rates. When the latter is not possible, the robots seek assistance from each other or human operators as shown in Section \ref{sec:help}. In Section \ref{sec:theory}, we summarize the theoretical performance guarantees of the proposed framework.
%\ref{sec:coorddescent}, we provide a decentralized planning method that leverages recent advances in Large Language Models (LLM) to design robot plans. In Section \ref{sec:cp}, we reason about the correctness of the designed plan with respect to the considered task using conformal prediction (CP). As in \cite{ren2023robots,wang2023conformal}, we also discuss how CP enables individual robots to ask on-the-fly for help from human operators when they are uncertain about correctness of their actions. 
The proposed algorithm is summarized in Alg. \ref{alg:MultiRobotLLM}. \textcolor{red}{[make sure that all refs to the algo lines appear in Section III-B too, since this where we discuss the overall algorithm.]}

% \textcolor{red}{[add refs to the algo lines throughout the text.]}


\subsection{A Centralized Planning Framework using LLMs}\label{sec:centralized}

%Existing (centralized or decentralized) multi-robot LLM-based planners to address Problem \ref{pr:pr1} often generate physically infeasible actions due to hallucinations of LLMs; see Section \ref{sec:intro}. This can be addressed by converting the mission planning problem into a multiple-choice question-answering (MCQA) problem as in \cite{ren2023robots,wang2023conformal,kumar2023conformal,ahn2022can}.
A potential solution to address Problem \ref{pr:pr1} is to directly apply the framework presented in \cite{ren2023robots} that is developed for single-robot task planning problems. The work in \cite{ren2023robots}, building upon \cite{ahn2022can,kumar2023conformal}, presents the task planning problem as a sequence of MCQA scenarios over time steps $t\in\{1,\dots,H\}$. In this setting, the question refers to the task $\phi$ along with a textual description of any possible mission progress. The choices refer to decisions $s_j(t)\in\ccalS$ that the (single) robot $j$ can make. Then, to pick the `best' action at time $t$, the LLM is queried $S=|\ccalS|$ times. A more detailed description can be found in \cite{ren2023robots}. This setting can be applied in the considered multi-robot planning problem by simply treating the multi-robot system as a single robot that can apply $N$ actions simultaneously. In this case, the number of choices/decisions $\bbs(t)$ in the MCQA framework are $S^N$. Thus, the employed LLM has to be queried $S^N$ times to pick a multi-robot action at a single time step $t$ which is impractical due to its token inefficiency. In fact, this can prohibitively increase the total API cost of using LLMs, especially, for long horizons $H$ or large number $N$ of robots. Also, the larger the number of choices in the MCQA framework is, the worse the planning performance gets, as shown by our empirical analysis. 

\begin{algorithm}[t]
\caption{Safe Planning for Language-instructed Robot Teams}\label{alg:MultiRobotLLM}
\begin{algorithmic}[1]
\State \textbf{Input}: NL task $\phi$; coverage guarantee $\alpha$; number of robots $N$; robot skills $\ccalA$; semantic environment $\Omega$
\State Initialize an ordered set $\ccalI=\{1, \dots, N\}$;\label{algo1:order_init}%$; 
\State Construct initial prompt $\ell_{\ccalI(1)}(t)$; decision set $\tau= \emptyset$; \label{algo1:prompt_init}
\For{$t=1~\text{to}~H$}
\For{$i\in\ccalI$}
\State Next robot $j=\ccalI(i)$
\State Compute the local prediction set $\mathcal{C}(\ell_j(t))$ %=\{s_j | g(s_j|\ell_j(t)) > 1-\bar{q} \}$ 
as in \eqref{eq:pred3local}\label{algo1:pred_set}
\If{ $|\mathcal{C}(\ell_j(t))|>1$ }
% \State Obtain new set $\ccalI = \ccalI'$ and restart algorithm
% \State Obtain help $s_j(t)$ from human operator \textcolor{red}{(our `help' function does more than this though by changing the order. add a couple more lines here. (the algo might get a bit complicated though..))}; \label{algo1:help}
\State Obtain help as in Section \ref{sec:help} \label{algo1:help}
\Else
\State  Pick the (unique) decision $s_j(t)\in\mathcal{C}(\ell_j(t))$
\EndIf
\State Construct $\bbs(t) = [s_1(t),\dots,s_N(t)]$
\State Append $\bbs(t)$ to the multi-robot plan $\tau$
\State Update $\ell_{I(i)+1}(t)=\ell_{j}(t)+s_j(t)+``\text{robot }\ccalI(i)+1"$ \label{algo1:prompt_update}
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}% \vspace{-0.5cm}
\normalsize

\subsection{Decentralized Multi-Robot Planning using LLMs}\label{sec:coorddescent}
%Our goal in this section is to design a planning algorithm capable of generating multi-robot mission plans $\tau$ accomplishing NL-expressed tasks $\phi$. We propose a coordinate descent-based planning algorithm that utilizes existing pre-trained LLMs to synthesize plans in a decentralized fashion. 
In this section, we propose a decentralized planning framework to address Problem \ref{pr:pr1} that is more token efficient than the one presented in Section \ref{sec:centralized}; see Remark \ref{rem:API}. Our setup leverages coordinate-descent methods that have been used extensively to address multi-robot planning problems in a decentralized manner \cite{atanasov2015decentralized,singh2009efficient}.
%allow the robots sequentially, as per some fixed order,  to design actions in a coordinate-descent manner. 
The key idea is that robots pick decisions at time $t$ successively (as opposed to jointly in Section \ref{sec:centralized}) using the MCQA setup, while incorporating the decisions of previous robots. In what follows, we describe our proposed decentralized planning algorithm in more detail.

%setting facilitating task reasoning and also significantly decreases the cost of using pre-trained LLMs. 



Consider a user-specified ordered set $\ccalI$ collecting the robot indices $j\in\{1,\dots,N\}$ where each robot index appears exactly once; e.g., $\ccalI=\{1,\dots,N\}$ [line \ref{algo1:order_init}, Alg. \ref{alg:MultiRobotLLM}]. We denote the $i-$th element in $\ccalI$ by $\ccalI(i)$. At each $t\in \{1\dots H \}$, the LLM will pick actions for each robot sequentially as per $\ccalI$. Specifically, robot $j=\ccalI(i)$ will select $s_j(t)$ while considering, all decisions that have been made until $t-1$, and all decisions made by the robots $\ccalI(1),\dots,\ccalI(i-1)$ at time $t$. Hereafter, for simplicity of notation, we assume that $\ccalI=\{1,\dots,N\}$ so that $\ccalI(j)=j$. %We note that such coordinate descent methods have been used to address various multi-robot planning problems in a more computationally efficient manner \cite{atanasov2015decentralized,singh2009efficient}.

%\begin{ex}[Feasible Plan Example(cont.)]
%As we have a homogeneous team of $3$ robots, the ordering is initialized as the ascending order of robot indices $I=[1, 2, 3]$. As shown in $\tau$, at $t=1$, $s_1(\text{go to}, \text{Pen},1)$ refers to the decision for robot $1$ made by the planner is `go to the location of Pen'; $s_2(\text{go to}, \text{Coke},1)$ refers to the decision for robot $2$ is `go to the location of Coke' given that robot $1$ was assigned to finish the task related to Pen; robot $3$ is not assigned to any task and set to idle given all the previous assignments for both robot $1$ and $2$. Similarly, at $t=2$, the planner will generate decisions sequentially based on $\ccalI$ and all the decisions made in $t=1$.
%\label{ex:me2} 
%\end{ex}

\textbf{Prompt Engineering:} In what follows, we discuss how each robot locally queries a pre-trained LLM to pick an action $s_j(t)$. The prompt used in this work consists of the following parts [line \ref{algo1:prompt_init}, Alg. \ref{alg:MultiRobotLLM}]. (1) \textit{System description} that defines the action space determining all possible actions $s_j(a,\bbx,t)$ that the robot can apply and rules that the LLM should always respect in its decision-making process. For instance, in our considered simulations, such rules explicitly determine that a robot cannot grasp an object located in a fridge before opening the fridge door. We observed that explicitly specifying such constraints improved the quality of LLM plans. We additionally require the length of the plan $\tau$ (i.e., the mission horizon) to be less than $H$, where $H\geq 0$ is a user-specified hyperparameter.
%
(2) \textit{Environment description} that describes the expected locations $\bbx_e$ of each semantic object $e$ of interest;
%
(3) \textit{Task description} that includes the task description $\phi$; 
%
(4) \textit{History of actions} that includes the sequence of actions, generated by the LLM, for all robots up to time $t-1$ and for all robots $1,\dots,j-1$ up to time $t$.
%
(5) \textit{Response structure} describing the desired structure of the LLM output for an example task.
%
(6) \textit{Current time step and robot index} describing the current time step $t$ and the index $j$ to the robot that is now responsible for picking an action as per $\ccalI$.

\textbf{Plan Design \& Execution:} Next, we describe how we use the above prompt to generate a feasible multi-robot plan $\tau$ incrementally. %so that our high-level task $\phi$ can be satisfied. 
The process of designing $\tau$ is converted into a sequence of $T>0$ MCQA scenarios for the LLM. Part $(4)$ in the above prompt does not include any textual information at time $t=0$. We denote the prompt associated with robot $j\in \ccalI$ at time $t$ by $\ell_j(t)$. %Also, we denote by $h(t, j)$ only part $(4)$ and $(6)$ of $\ell(t,j)$. 
Given $\ell_j(t)$ and $\ccalI$, the LLM is asked to select a decision $s_j(t)$, for robot $j$, among all available ones included in part (1). Given any $s_j(t)\in \mathcal{S}$, LLMs can provide a score $r(s_j(t)|\ell(t))$; the higher the score, the more likely the decision $s_j(t)$ is a valid next step to positively progress the task. To get the scores $r(s_j(t)|\ell(t))$ for all $s_j(t)\in \mathcal{S}$, we query the model over all potential decisions $s_j$ (i.e., $S=|\ccalS|$ times in total). Then, we convert them into a vector of normalized scores using the softmax function. We denote the softmax score of a decision $s_j$ by $g(s_j|\ell_j(t))$. 

Using these softmax scores, a possible approach to select the $s_j$ is by simply choosing the decision with the highest softmax score, i.e., $s_j(t)=\arg\max_{s_j\in\mathcal{S}} g(s_j|\ell_j(t))
$, as e.g., in \cite{ahn2022can}. However, this point-prediction approach is uncertainty-agnostic; note that these softmax scores do not represent calibrated confidence \cite{ren2023robots}. A much preferred approach would be to generate set predictions, denoted by $\ccalC(\ell_j(t))$ that contain the ground truth action with a user-specified high-probability. Hereafter, we assume that such prediction sets are provided; we defer their construction, using CP, to Section \ref{sec:cp} (see \eqref{eq:pred3local}). Given $\ccalC(\ell_j(t))$, we select decisions $s_j(t)$ based on the following two cases. If $\ccalC(\ell_j(t))$ is singleton, then we select the action included in $\ccalC(\ell_j(t))$ as it contributes to mission progress with high probability.\footnote{By construction of the prediction sets, this action coincides with $s_j(t)=\arg\max_{s_j\in\mathcal{S}} g(s_j|\ell_j(t))$; see Section \ref{sec:cp}}. Otherwise, robot $j$ seeks assistance from its teammates and/or a human operator to select $s_j(t)$. The latter is discussed in Section \ref{sec:help}.

%\begin{equation}
%s_j(t)=\arg\max_{s_j\in\mathcal{S}} g(s_j|\ell_j(t)).
%\end{equation}


Once $s_j(t)$ is selected, we record $s_j(t)$ into part $(4)$ and also update part $(6)$ by putting the next robot index $j+1$ based on the ordering $\ccalI$ into the prompt. With slight abuse of notation, we denote the prompt update by $\ell_{j+1}(t) = \ell_{j}(t) + s_j(t) + \text{`robot~$j+1$'},$ where the summation means concatenation of text [line \ref{algo1:prompt_update}, Alg. \ref{alg:MultiRobotLLM}]. We repeat the above procedure sequentially over all robots $j$ as per $\ccalI$. This way, we construct the multi-robot action $\bbs(t)$.
% here add the multi-robot setup 
Once $\bbs(t)$ is constructed, the robots execute their corresponding actions simultaneously, and the current time step is updated to $t+1$ in part (6).  Part (4) and (6) are being updated during the time interval $[t+1, t+H-1]$.  The above process is repeated to design $\bbs(t+1)$ only when all robots have completed execution of $s_j(t)$. This way, we generate a plan $\tau=\bbs(1),\dots,\bbs(t),\dots,\bbs(H)$ of horizon $H$. %We remark that robot $j$ cannot execute the next action $s_{$
%Here as the length of each $S(t)$ is $N$, the plan $\tau$ is comprised of $T=H\times N$ decisions where each robot $i\in I$ will have its own decision set of $\{ s_i(0), s_i(1), \dots, s_i(H-1) \}$ corresponding to the trajectory this robot should follow. For a high-level task $\phi$ with $K\geq 1$ sub-tasks, we let LLMs reason about the current status of task assignment based on the prompt and generate decisions for each robot in the team.



\begin{rem}[Unknown \& Dynamic Environments]
    Recall from Section \ref{sec:problem} that we consider  environments where the locations of the semantic objects are known and fixed over time. To account for dynamic environments, at every time step $t$, once the multi-robot action $\bbs(t)$ is computed and executed, part (2) in the prompt should be updated to account e.g., for new or any missing objects.
\end{rem}

\begin{rem}[Token Efficiency Benefits]\label{rem:API}
    Observe that the number of choices/decisions $s_j(t)$ in the MCQA framework is $S$. Thus, to design the multi-robot action $\bbs(t)$, the LLM is queried $N\cdot S$ times, which is significantly smaller than $S^N$ required in the centralized approach in discussed Section \ref{sec:centralized}. This allows us to design multi-robot plans in a more token-efficient way, and mitigate the API costs incurred in the centralized setting which increase exponentially as the number of robots increases.
\end{rem}

\subsection{Decentralized Uncertainty Quantification using CP}\label{sec:cp}

In this section, we discuss how the prediction sets $\ccalC(\ell_j(t))$, introduced in Section \ref{sec:coorddescent}, are constructed, given a required task success rate $(1-\alpha)$\% (see Problem \ref{pr:pr1}). %As it will be shown in Section \ref{sec:theory}, these prediction sets allow us to characterize the task success rate of the proposed planner.
%
%A key challenge lies in reasoning about the correctness of plan $\tau$ with respect to $\phi$. To address this challenge, 
In what follows, inspired by \cite{ren2023robots}, we employ conformal prediction (CP) to construct these prediction sets. %to compute a prediction set that contains plans that satisfy the high-level task $\phi$ with high probability. Later, we show how to use this prediction set to reason about mission satisfaction. 
To better illustrate the challenges of their construction, we consider the following cases (that build upon each other): (i) single-robot \& single-step plans %(ii) multi-robot \& single-step plans; 
and (ii) multi-robot \& multi-step plans.

\textbf{Single-robot \& Single-step Plans:} Initially, we focus on cases where $N=1$ and on tasks $\phi$ that can be satisfied by plans $\tau$ with $H=1$. Later we generalize the results for $H\geq 1$ and $N\geq 1$. 
%
First, we collect a calibration dataset $\ccalM=\{(\ell_{j,\text{calib}}^i,\tau_{\text{calib}}^{i})\}_{i=1}^M$, using data drawn from $\ccalD$, where $\ell_{j,\text{calib}}^i$ is the prompt corresponding to the single robot $j$ for a task $\phi_i$ and $\tau_{\text{calib}}^{i}=s_{j,\text{calib}}^{i}(1)$ is the corresponding ground truth decision for robot $j$. Hereafter, we drop the dependence of the robot decisions on the time step, since we consider single-step plans. %Similarly, notice that we dropped the dependence of the prompt on the robot indices since we consider a single robot.
%
We assume that there exists a unique correct decision $s_{j,\text{calib}}^{i}$ for each $\ell_{j,\text{calib}}^i$. %This assumption can be relaxed exactly as in [CITE]. 
This assumption can be relaxed as in \cite{ren2023robots}; due to space limitations we abstain from this presentation.
%


Consider a new test data point $\ell_{j,\text{test}}$ (corresponding to a task $\phi_{\text{test}}$), drawn from $\ccalD$, %(denoted by $\ell(0)$ earlier) 
with unknown correct decision $s_{j,\text{test}}$ for robot $j$. CP can generate a prediction set $\ccalC(\ell_{\text{test}})$ of decisions $s_j$ containing the correct one $s_{j,\text{test}}$ with probability greater than $1-\alpha$, i.e., 
%
%
\begin{equation}\label{eq:CP1}
P(s_{j,\text{test}}\in \mathcal{C}(\ell_{j,\text{test}})) \geq 1-\alpha,
\end{equation}
where $\alpha\in[0,1]$ is user-specified.
%
To generate $\mathcal{C}(\ell_{j,\text{test}})$, CP first uses the LLM’s confidence $g$ to compute the set of
non-conformity scores (NCS) $\{r^i=1-g(s_{j,\text{calib}}^i~|~\ell_{j,\text{calib}}^i)\}_{i=1}^M$ over the calibration set.
%
The higher the score is, the less each data in the calibration set conforms to the data used for training the LLM. Then CP performs calibration by computing the $\frac{\ceil{(M+1)(1-\alpha)}}{M}$ empirical quantile of $r_1,\dots,r_M$ denoted by $q$. Then, it generates the prediction set 

\begin{equation}\label{eq:pred1}
\mathcal{C}(\ell_{j,\text{test}})=\{s_j\in \ccalS~|~g(s_j|\ell_{j,\text{test}})>1-q\},
\end{equation}
%
that includes all labels (i.e., decisions) that the predictor is at least $1-q$ confident in. This prediction set should be should be used to select decisions as per Section \ref{sec:coorddescent} for single-robot single-step tasks. 

The generated prediction set ensures that the $1-\alpha$ \textit{marginal} coverage guarantee, mentioned above, holds. By construction of the prediction sets the decision $s_j=\arg\max_{s_j\in\mathcal{S}} g(s_j|\ell_{j,\text{test}})$ belongs to $\mathcal{C}(\ell_{j,\text{test}})$. A key requirement in CP is that all calibration and test data points are i.i.d. which holds in this setup by assumption; see Problem \ref{pr:pr1}. 







\textbf{Multi-robot \& Multi-step Plans:} Finally, we generalize the above result to the general case where $N\geq1$ and $H\geq 1$.
%multi-robot case (i.e., $N\geq 1$) where the accomplishing ta $\phi$ requires plans $\tau$ with $T > 1$ decisions selected from $\ccalS$. Here notice that $T>1$ may refer to a) single-robot-multi-step ($H>1, N=1$); b) multi-robot-single-step ($H=1, N>1$); or c) multi-robot-multi-step ($H>1, N>1$). 
%
%Observe that we cannot apply \eqref{eq:localPred2} to compute  local prediction sets $\ccalC(\ell_{j,\text{test}}(t))$ associated with robot $j$ at every time step $t$.
Notice that here we cannot apply directly \eqref{eq:CP1}-\eqref{eq:pred1} to compute individual prediction sets $\ccalC(\ell_{j,\text{test}}(t))$ for each robot $j$ given a new task $\phi_{\text{test}}$, which violates the i.i.d. assumption required to apply CP. %In fact, the distribution of prompts $\ell_{j,\text{test}}(t)$ depends on  decisions that have already been selected by the robots $1,\dots,j-1$ at time $t$. 
In fact, the distribution of prompts $\ell_{j,\text{test}}(t)$ depends on the previous prompts i.e., the multi-robot decisions at $t'<t$ as well as the decisions of robots $1,\dots,j-1$ at time $t$. 
%
To address this challenge, the key idea is to (i) lift the data to sequences, and (ii) perform calibration at the sequence level using a carefully designed nonconformity score function. %Hereafter, we drop the dependence on $t$, since we focus on single-step plans.

%The challenge in this case is that the test points $\{(\ell_{\text{test}}(t+k,j),\bbs_{\text{test}}(t+k))\}_{k=1}^H$ are not independent with each other. 
%
%The reason is that the distribution of prompts $\ell_{j,\text{test}}(t)$ depends on the previous prompts i.e., the multi-robot decisions at $t'<t$ as well as the decisions of robots $1,\dots,j-1$ at time $t$. 
%To address this challenge, we will perform a similar analysis as in the previous case by performing calibration at the sequence level.

First, we construct a calibration dataset as follows [line \ref{algo1:cp}, Alg. \ref{alg:MultiRobotLLM}]. We generate $M\geq1$ high-level tasks $\phi_i$ defined over various number of robots $N_i$ and mission horizons $H_i$. Each task $\phi_i$ is broken into a sequence of $T=H_i\cdot N_i\geq 1$ prompts.%where $H_i$ is a task horizon associated with $\phi_i$.
\footnote{
%
%We assume that the calibration sequences \eqref{eq:prompt2cal}-\eqref{eq:plan2cal} are sampled from the (unknown) distribution $\ccalD$, introduced in Problem \ref{pr:pr1} \cite{ren2023robots}. Observe also that that these sequences share the same order of indices as per an ordered set $\ccalI_i$ (sampled from $\ccalD$ as part of $\phi_i$). Note that these ordered sets do not need not be the same across the calibration sequences. For simplicity of notation, in \eqref{eq:prompt2cal}-\eqref{eq:plan2cal}, we assume that that $\ccalI_i=\{1,\dots,N\}$ for all sequences $i$; we make the same assumption for the test sequence as well.
%
We assume that the  sequences \eqref{eq:seqProm}-\eqref{eq:Plans3}, along with $N_i$, are sampled from the (unknown) distribution $\ccalD$, introduced in Problem \ref{pr:pr1}. Essentially, we assume that a task $\phi$ in a scenario $\xi$ appears as a sequence of prompts as defined in \eqref{eq:seqProm}.
%
Observe also that these sequences share the same order of robot indices as per an ordered set $\ccalI_i$ (sampled from $\ccalD$ as part of $\phi_i$). Note that these ordered sets do not need not be the same across the calibration sequences. 
%This implies that the scenarios sampled from $\ccalD$ include also the number $N_i$ of robots as well as the ordered set $\ccalI_i$. As before, only 
For simplicity of notation, we assume that $\ccalI_i=\{1,\dots,N_i\}$ for all sequences $i$; we make the same assumption for the test sequence as well.} This sequence of $T$ prompts is denoted by
%
\begin{align}\label{eq:seqProm}
&\bar{\ell}_{\text{calib}}^i=\underbrace{\ell_{1,\text{calib}}^i(1),\dots,\ell_{j,\text{calib}}^i(1),\dots,\ell_{N_i,\text{calib}}^i(1)}_{t=1},\dots,\nonumber\\&
%
\underbrace{\ell_{1,\text{calib}}^i(t'),\dots,\ell_{j,\text{calib}}^i(t'),\dots,\ell_{N_i,\text{calib}}^i(t')}_{t=t'},\dots,\nonumber\\&
%
\underbrace{\ell_{1,\text{calib}}^i(H_i),\dots,\ell_{j,\text{calib}}^i(H_i),\dots,\ell_{N_i,\text{calib}}^i(H_i)}_{t=H_i}.
\end{align}
%
Then, as before, for each prompt $\bar{\ell}_{\text{calib}}^i$, we  manually construct the corresponding sequence of ground truth decisions:
%
\begin{align}\label{eq:Plans3}
&\tau_{\text{calib}}^i=\underbrace{s_{1,\text{calib}}(1),\dots,s_{j,\text{calib}}(1),\dots,s_{N_i,\text{calib}}(1)}_{=\bbs(1)},\dots,\nonumber\\&
\underbrace{s_{1,\text{calib}}(t'),\dots,s_{j,\text{calib}}(t'),\dots,s_{N_i,\text{calib}}(t')}_{=\bbs(t')},\dots,\nonumber\\&
\underbrace{s_{1,\text{calib}}(H_i),\dots,s_{j,\text{calib}}(H_i),\dots,s_{N_i,\text{calib}}(H_i)}_{=\bbs(H_i)}.
\end{align}
%
\noindent
This gives rise to a calibration set  $\ccalM=\{(\bar{\ell}_{\text{calib}}^i,\tau_{\text{calib}}^i)\}_{i=1}^M$ constructing by drawing i.i.d. samples from $\ccalD$.
%
%Notice that the prompts were built sequentially as per the coordinate descent method. Hence with a horizon of $H_i$ for task $\phi_i$, the sequence of prompts $\bar{\ell}_{\text{calib}}^i$ can be  rewritten into the form of 
%\begin{equation}
%\bar{\ell}_{\text{calib}}^i = 
%[L_{\text{calib}}^i(0),\dots, L_{\text{calib}}^i(H_i-1)]
%\end{equation}
%\noindent 
%where $L_{\text{calib}}^i(t) = \{ \ell_{\text{calib}}^{i, j}(t) \}, \forall j\in I_{N_i}$ refers to the prompts for each robot $j$ at time step $t$.
%
%Also, ground truth decision sequence can be written as 
%\begin{equation}
%\tau_{\text{calib}}^i=S_{\text{calib}}^i(0),\dots,S_{\text{calib}}^i(H_i-1),
%\end{equation}
%\noindent
%where $S_{\text{calib}}^i(t) = \{ s_{\text{calib}}^{i, j}(t) \}, \forall j \in I_{N_i}$. Here each time step $t$ will include $N_i$ prompts and decisions corresponding to all robots in the team.
%
As before, we assume that each context $\bar{\ell}_{\text{calib}}^i$ has a unique correct plan $\tau_{\text{calib}}^i$.
%
Hereafter, we denote by $\bar{\ell}_{\text{calib}}^i(k)$ and $\tau_{\text{calib}}^i(k)$ the $k$-th entry in the sequences $\bar{\ell}_{\text{calib}}^i$ and $\tau_{\text{calib}}^i$, respectively for the sake of simplicity, where $k\in\{1,\dots,T\}$. 

\begin{rem}[Sequence Element Index]
We emphasize that $k$ is different from the time step $t\in\{1,\dots,H_i\}$ and $T$ is the same across all calibration points, such that for any datapoint with index $i\in \{1, \dots, M \}$, we can always find a corresponding index $k$ denoted as $\bar{\ell}^i(k)$ that is equivalent to the $j$-th robot at time step $t$ denoted as $\ell^i_{j}(t)$.
\end{rem}


Next, for each calibration datapoint, we define the NCS similarly to the multi-robot-single-step plan case. Particularly, the score of a decision $\tau_{\text{calib}}^i(k)$ is $r_k^i=1-g(\tau_{\text{calib}}^i(k)~|~\bar{\ell}_\text{calib}^i(k))$, for all $k\in\{1,\dots,T\}$ (as defined in the single-robot \& single step plan case). Then, the NCS of the multi-robot plan $\tau_{\text{calib}}^i$ is the lowest score over $k\in\{1,\dots,T\}$, i.e., 
%
\begin{equation}\label{eq:min_seqpred}
\bar{g}(\tau_{\text{calib}}^i~|~\bar{\ell}_\text{calib}^i)=\min_{k\in\{1,\dots, T\}}g(s_\text{calib}^i(k)~|~\bar{\ell}_\text{calib}^i(k)).
\end{equation}
%
Thus, the NCS of each calibration sequence $i$ is
\begin{equation}
\bar{r}_i=1-\bar{g}(\tau_{\text{calib}}^i|\bar{\ell}_\text{calib}^i).
\end{equation}

Consider a new scenario drawn from $\ccalD$ associated with a task $\phi_{\text{test}}$ that is defined over $N_{\text{test}}$ robots and corresponds to a sequence of prompts $\bar{\ell}_{\text{test}}=\bar{\ell}_{\text{test}}(1),\dots,\bar{\ell}_{\text{test}}(k),\dots,\bar{\ell}_{\text{test}}(T)$ with unknown correct label/plan $\tau_{\text{test}}$. We select the mission horizon $H_\text{test}\geq 1$ so that $T=H_\text{test}\cdot N_{\text{test}}$.
%
Using CP, we can generate a prediction set $\bar{\ccalC}(\bar{\ell}_{\text{test}})$ of plans $\tau$ containing the correct one $\tau_{\text{test}}$  with high probability i.e., %{\phi,\text{test}}
\begin{equation}\label{eq:CP3}
P(\tau_{\text{test}}\in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}})) \geq 1-\alpha,
\end{equation}
where the prediction set $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is defined as [line \ref{algo1:pred_set}, Alg. \ref{alg:MultiRobotLLM}] 
%
\begin{equation}\label{eq:pred3}
\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\{\tau~|~\bar{g}(\tau| \bar{\ell}_{\text{test}})>1-\bar{q}\}, 
\end{equation}
%
where $\bar{q}$ is the $\frac{(M+1)(1-\alpha)}{M}$ 
%
empirical quantile of $\bar{r}_1,\dots,\bar{r}_M$. The generated prediction set ensures that the coverage guarantee in \eqref{eq:CP3} holds. %By construction of the prediction sets, the plan $\tau$ generated by the LLM belongs to $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$. 
%
The size of the prediction sets can be used to evaluate uncertainty of the LLM. Specifically, if $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is singleton then this means that the LLM is certain with probability at least $1-\alpha$ that the designed multi-robot accomplishes the assigned task.
%

\underline{On-the-fly and Local Construction:}
Observe that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ in \eqref{eq:pred3} is constructed after the entire sequence $\bar{\ell}_{\text{test}}=\bar\ell_{\text{test}}(1),\dots,\bar\ell_{\text{test}}(T)$ is observed. %This means uncertainty quantification of the LLM can be performed only after the whole plan is designed. %This may limit applicability of the proposed framework in offline missions.
%However, at every (test) time $t\in\{1,\dots,H_{\text{test}}\}$, the robot
%
%does not see the entire sequence $\bar{\ell}_{\text{test}}$ all at once; instead at every time $t\in\{1,\dots,H_{\text{test}}\}$
%observes only $\ell_{\text{test}}(t)$ and not the whole sequence. 
%Similarly to the previous case, next we discuss how the prediction set can be constructed on-the-fly.
%
This means uncertainty quantification of the LLM can be performed only after the whole plan is designed. %This may limit applicability of the proposed framework in offline missions.
%However, at every (test) time $t\in\{1,\dots,H_{\text{test}}\}$, the robot
%
%does not see the entire sequence $\bar{\ell}_{\text{test}}$ all at once; instead at every time $t\in\{1,\dots,H_{\text{test}}\}$
%observes only $\ell_{\text{test}}(t)$ and not the whole sequence. 
However, at test time, we do not see the entire sequence of prompts all at once; instead, the contexts $\bar{\ell}_{\text{test}}(k)$ are revealed sequentially, one at a time. We thus need to construct the prediction set on-the-fly, using only the current and past information, as the robots take turns in querying the LLM for action selection.
%
At every iteration $k\in\{1,\dots,T\}$, we construct the local prediction set associated with a robot $j$ and a time step $t$,  
\begin{equation}\label{eq:pred3local}
    \mathcal{C}(\bar{\ell}_{\text{test}}(k)))=\{\tau_{\text{test}}(k)~|~g(\tau_{\text{test}}(k)|\bar{\ell}_{\text{test}}(k)))>1-\bar{q}\},
\end{equation}
where $g$ refers to the softmax score used in Section \ref{sec:coorddescent}. This prediction set should be used to select robot decisions $s_j(t)$ as discussed in Section \ref{sec:coorddescent}. Also, notice that
%generalizes the prediction sets \eqref{eq:pred1} and \eqref{eq:localPred2} to multi-robot and multi-step plans. In other words, 
\eqref{eq:pred3local} degenerates to \eqref{eq:pred1} if $H_{\text{test}}=1$ and $N_{\text{test}}=1$.
%
%Alternatively, %as in our implementation in Section \ref{sec:experiments},  
%$\mathcal{C}(\ell(t)))$ can be constructed using the RAPs approach that can result in smaller prediction sets \cite{angelopoulos2020uncertainty}; see Section \ref{sec:predSet}.
%
%
%Then, the causal prediction set associated with $\bar{\ell}_{\text{test}}$ is defined as  
%
% $\mathcal{C}(\bar{\ell}_{\text{test}})=\mathcal{C}(\ell(0)))\times\mathcal{C}(\ell(1)))\dots\mathcal{C}(\ell(H_{\text{test}})))$. 
%
%
%
As it will be shown in Section \ref{sec:theory}, it holds that 
\begin{equation}\label{eq:causalPred3}
\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}(0)))\times\mathcal{C}(\bar{\ell}(1)))\dots\mathcal{C}(\bar{\ell}(k)))\dots\times\mathcal{C}(\bar{\ell}(T))).
\end{equation}

% \begin{equation}\label{eq:causalPred3}
% \bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\ell(0)))\times\mathcal{C}(\ell(1)))\dots\mathcal{C}(\ell(k)))\dots\times\mathcal{C}(\ell(T))).
% \end{equation}


As it will be discussed in Section \ref{sec:help}, this causal construction of the prediction sets allow us to identify on-the-fly, i.e., as the multi-robot plan is constructed, for which robot $j$ and at what time step $t$, the LLM is uncertain about the correct decisions. This is particularly important for real-time missions where the robots should execute their decisions $s_j(t)$ as soon as they are made.

\begin{rem}[Communication Architecture]

The approach for the construction of the prediction set 
$\bar{\ccalC}(\bar{\ell}_{\text{test}})$ in \eqref{eq:causalPred3} is not fully-distributed because multi-hop
communication is needed to pass information across robots. However, all-to-all communication is not required either because the construction of the prediction sets and, consequently, the decision making process (Section \ref{sec:coorddescent}) naturally occurs in communication hops. 
%
To construct the prediction sets and select decisions $s_j(t)$, the robots should transmit to each other their current decisions in order to compute the history of actions required to construct part (4) in the prompt $\bar{\ell}_{\text{test}}$; see Section \ref{sec:coorddescent}.
%    
\end{rem}


% \begin{rem} [Dataset-Conditional Guarantee]\label{rem:datasetInd}
% The probabilistic guarantee in \eqref{eq:CP3} is \textit{marginal} in the sense that the probability is over both the sampling of the calibration set $\ccalM$ and the test point $\ell_{\text{test}}$. Thus, a new calibration set will be needed for every single test data point $\bar{\ell}_{\text{test}}$ to ensure the desired probability $1-\alpha$, which is not practical. Thus, as in \cite{vovk2012conditional,ren2023robots}, we can apply the following dataset-conditional guarantee which holds for a fixed calibration set:
% %
% \begin{equation}\label{eq:data_cond_guarantee}
% P(\tau_{\text{test}}\in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}}) | \ccalM) \geq \text{Beta}^{-1}_{M+1-v, v}(\delta),
% \end{equation}
% \noindent
% where $\text{Beta}^{-1}_{M+1-v, v}(\delta)$ denotes the quantile level of $\delta$ in a Beta distribution with $v= \left \lfloor{(M+1)\alpha_{\ccalM})}\right \rfloor$. 
% %
% Given a calibration dataset of size $M$ and a small value for $\delta$ ($\delta=0.01$), to achieve the desired coverage guarantee $1-\alpha$ (with probability $1-\delta$), we compute the parameter $\alpha_{\ccalM}$ so that $\alpha = 1- \text{Beta}^{-1}_{M+1-v, v}(\delta)$.
% \end{rem}


\subsection{Seeking Assistance from Teammates and Human Operators}
\label{sec:help}

%\textbf{Ask-for-Help:} 
As discussed in Section \ref{sec:coorddescent}, if $\mathcal{C}(\bar{\ell}(k)))$ is singleton, then this means that the LLM is certain that the decision $s_j(t)$ included in  $\mathcal{C}(\bar{\ell}(k)))$ will contribute to making mission progress. Otherwise, the corresponding robot seeks assistance in two ways [line \ref{algo1:help}, Alg. \ref{alg:MultiRobotLLM}]. First, a message is sent to all previous robots asking them to re-plan their actions for the time step $t$ but in a different order $\ccalI$.
%we change the $\ccalI$ and ask the robots to re-plan their actions for the current time-steps, 
We iterate over various ordered sets $\ccalI$ until singleton prediction sets are generated for all robots.\footnote{Notice that this step may be computationally expensive to perform online and it may also increase the cost of using LLMs. Thus, it may be neglected for large robot teams and action spaces. %\textcolor{red}{[we can delete the following, as it is kinda repetitive, once you confirm you agree with it]} Also, notice %that quantile $\bar{q}$ used to compute the prediction sets may depend on $\ccalI$; 
%that given a fixed task $\phi$, different ordered 
%order sets $\ccalI$ will yield different sequences of prompts in \eqref{eq:seqProm}. This may result in different NCS for calibration sequences, and, consequently, in a different quantile $\bar{q}$ (for a fixed $1-\alpha$). Thus, a test-time sequence of prompts $\bar{\ell}_{\text{test}}$ constructed using $\ccalI$ that is different from the one used in the construction of the calibration dataset may violate the i.i.d. assumption required to apply CP. This in turn may invalidate the provided coverage guarantees (although this is challenging to formally prove). This can be mitigated by considering calibration data points of various, instead of fixed, ordered sets $\ccalI$.
%
%
%changing the order in $\ccalI$ at test time does not violate the coverage guarantees discussed in Section \ref{sec:cp}, as long as the distribution $\ccalD$ can generate tasks (i.e., sequences of prompts $\bar{\ell}_{\text{test}}$ defined in Section \ref{sec:cp}) as per the new order $\ccalI$. Otherwise, changing the order in $\ccalI$ may violate the i.i.d. assumption required to apply CP (although this is challenging to formally prove).
} Our empirical analysis has shown that $\ccalI$ can affect the size of prediction sets; see Section \ref{sec:experiments}. Observe that by changing the ordered set $\ccalI$, we essentially switch to a different test scenario $\xi$ (since $\ccalI$ is considered part of the task $\phi$) that may correspond to a different prediction set. However, the new and the previous scenario are semantically the same, as they both refer to the same language-based mission. Therefore, in practice, it does not matter for which of these scenarios (that differ only in the ordered set $\ccalI$) a plan is computed.
%
If such a set $\ccalI$ cannot be found with the next $I$ attempts, for some user-specified $I>0$, the robots request help from human operators as in \cite{ren2023robots}. Particularly, the robot presents to a user the set $\mathcal{C}(\bar{\ell}(k)))$ (along with the prompt $\bar{\ell}(k)$) and asks them to choose one action from it. The operator either picks an action for the corresponding robot or decides to halt operation.

%\begin{rem}[CP \& Dynamic Order $\ccalI$]
%\textcolor{red}{[maybe we should remove this...]}
%We note here that changing the order of robot indices in  $\ccalI$ at test-time would violate the coverage guarantees provided in Section \ref{sec:cp} if the robots were heterogeneous in their skills. The reason is that this may switch the ground truth plans/labels in the calibration dataset from feasible to infeasible (which is not the case in the considered homogeneous robot case). Consequently, this would change the quantiles used to construct the prediction sets.  
%Notice that changing the order in $\ccalI$ at test time does not violate the coverage guarantees, as long as the distribution $\ccalD$ can generate tasks (i.e., sequence of prompts $\bar{\ell}_{\text{test}}$ defined in Section \ref{sec:cp}) as per the new order. Otherwise, changing the order in $\ccalI$ may violate the i.i.d. assumption required to apply CP.
%\end{rem}


\subsection{Theoretical Guarantees for Mission Success Rate}\label{sec:theory}
 
% \textcolor{red}{[put here two results. One about the causal prediction and one about the mission success rates. It's fine to say that the proofs are similar to the ones in princeton and that we present them here for completeness of the paper]}

% \textcolor{red}{[You need to carefully read what you have written in this section. There are several mistakes. For instance in the proposition you want to show that these two prediction sets (let’s call them A and B) are equivalent. This means that you need to show that if x belongs to A, it also belongs to B, and vice versa (that’s the purpose of the $\leftrightarrow$ symbol in the proposition statement). Your current proof seems to be addressing only one direction. If the other direction is straightforward or if the steps in the proof hold for the other direction, you need to acknowledge it and provide a brief explanation. Also, there are several notational issues here. Make sure there are no incorrect or undefined symbols. I have made such comments a couple of times in your drafts, try to be more careful. ]}

\begin{prop}\label{prop:eq_prop}
$\tau_{\text{test}} \in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}}) \Leftrightarrow \tau_{\text{test}} \in \mathcal{C}(\bar{\ell}_{\text{test}})$
\end{prop}

\begin{proof}
This proposition follows from \eqref{eq:min_seqpred} and \eqref{eq:pred3}.
$\tau_{\text{test}} \in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is equivalent to $\min_{k=\{1,\dots,T\}} g(s_{\text{test}}(k) | \bar{\ell}_{\text{test}}(k) )>1-\bar{q}$. Then we can infer $\min_{k=\{1,\dots,T\}} g(s_{\text{test}}(k) | \bar{\ell}_{\text{test}}(k) )>1-\bar{q} \Leftrightarrow \forall k\in \{1,\dots,T\}, g(s_{\text{test}}(k) | \bar{\ell}_{\text{test}}(k) )>1-\bar{q}$. From \eqref{eq:pred3local}, we can construct $\mathcal{C}(\bar{\ell}_{\text{test}}(k))$, and compute the product of $\mathcal{C}(\bar{\ell}_{\text{test}}(k))$ for all $k\in \{1,\dots,T\}$ such that $\bar{\ell}_{\text{test}} \in \mathcal{C}(\bar{\ell}_{\text{test}})$ completing the proof.

% If $\bar{\ell}_{\text{test}} \in \bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$, then $\min_{k=\{1,\dots,T\}}g(s_{\text{test}}(k) | \ell_{\text{test}}(k) )>1-\bar{q}$. Such that for any $k\in \{1,\dots,T\}$, we have $g(s_{\text{test}}(k) | \ell_{\text{test}}(k) )>1-\bar{q}$. Then we can infer from \eqref{eq:pred3local} that  $\bar{\ell}_{\text{test}} \in \mathcal{C}(\bar{\ell}_{\text{test}})$ completing the proof.
\end{proof}

% \textcolor{red}{[here you need to add a proposition stating that the causally constructed prediction set is the same as the non-causal one. (The following text has already been included earlier.) You also need a proof for that. I am pretty sure it's just one line and probably the same as in the princeton paper but it has to be stated here]}
% \textbf{Causal Construction of Prediction Set:} Observe that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$ is constructed after the entire sequence $\bar{\ell}_{\text{test}}$ is observed. 
% %
% However, at every step $k\in \{1,\dots,T \}$, the LLM observes only $\bar{\ell}_{\text{test}}(k)$ and not the whole sequence. Thus, the prediction set needs to be constructed in a causal manner using only the current and past information. Thus, at every step $k$, we construct the causal prediction set  $\mathcal{C}(\bar{\ell}_{\text{test}}(k)))=\{s~|~g(s|\bar{\ell}_{\text{test}}(k)))>1-\bar{q}\}$. 
% %
% Then, the causal prediction set associated with $\bar{\ell}_{\text{test}}$ is defined as  $\mathcal{C}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}_{\text{test}}(1)))\times\mathcal{C}(\bar{\ell}_{\text{test}}(2)))\dots\mathcal{C}(\bar{\ell}_{\text{test}}(T)))$. As shown in \cite{ren2023robots}, $\mathcal{C}(\bar{\ell}_{\text{test}})$ and $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})$, it holds that $\bar{\mathcal{C}}(\bar{\ell}_{\text{test}})=\mathcal{C}(\bar{\ell}_{\text{test}})$.


\textcolor{red}{[the next theorem does not add anything new. we have shown this in the cp section. we need to replace it with a theorem about the mission success rate as in the pricneton paper. After all, problem 1, says that we want our planner to achieve desired success rates]}
\textbf{Probabilistic LTL Satisfaction Guarantees:} Using the above CP framework, we can state the following result. 

% \textcolor{red}{[you need to clean up the following result- no LTL, no $\models$ etc]}
\begin{theorem}\label{thm1}
The completion rate over new (but i.i.d.) test scenarios $\phi_{\text{test}}$ is at least $1-\alpha$, if $|\mathcal{C}(\bar{\ell}_{\text{test}}(k)))|=1$, for all $k\in\{1,\dots,T\}$ i.e.,
$\mathbb{P}(\tau_{{\text{test}}}\in \mathcal{C}(\bar{\ell}_{\text{test}})\geq 1-\alpha$.
\end{theorem}

\begin{proof}
This result follows directly from \eqref{eq:CP3}.
If $|\mathcal{C}(\bar{\ell}_{\text{test}}(k))|=1$, for all $k\in\{1,\dots,T\}$, then using proposition \ref{prop:eq_prop},  we have that \eqref{eq:CP3} is equivalent to $\mathbb{P}(\tau_{{\text{test}}}\in \mathcal{C}(\bar{\ell}_{\text{test}})\geq 1-\alpha$ %(with probability $1-\delta$ as discussed in Remark \ref{rem:datasetInd})
%
, completing the proof.
\end{proof}

==> problem.tex <==
\section{Problem Formulation}


\subsection{Robot System and Skills}\label{sec:robot}

Consider a team of $N$ homogeneous mobile robots where each robot $i=\{1, 2, \dots, N\}$ is governed by the same following dynamics: $\bbp(t+1)=\bbf(\bbp(t),\bbu(t))$, where $\bbp(t)\in\ccalP\subset\mathbb{R}^m$ stands for the state (e.g., position and orientation) of the robot, and $\bbu(t)\in\mathbb{R}^b$ stands for control input at discrete time $t$. We assume that for every robot $i$ state $\bbp_i(t)$ is known for all time instants $t\geq0$.
%
Every robot in the team shares the same number of $A>0$ abilities/skills collected in a set $\ccalA\in\{1,\dots,A\}$. Each skill $a\in\ccalA$ is represented as text such as `take a picture', `grab', or `move to'. Application of a skill $a$ at an object/region with location $\bbx$ at time $t\geq0$ is denoted by $s_i(a,\bbx,t)$ for robot $i$. In this paper, we consider homogeneous robots such that at time $t\geq0$ for all possible objects/regions $\bbx$ considered in the environment, every robot in the team can achieve the same application set of skills such that $\{ s_i(a, \bbx, t)\}$ is equivalent for all robot $i$. With slight abuse of notation, when it is clear from the context, we denote by $s(t)$ for brevity
%
Also, we assume that every robot in the team has access to low-level controllers $\bbu(t)$ to apply the skills in $\ccalA$. Hereafter, we assume perfect/error-free execution of these capabilities.

\subsection{Semantic Environment}

The entire team of robots resides in a semantic environment $\Omega\subseteq \mathbb{R}^d, d\in\{2,3\}$ with fixed, static, and known obstacle-free space denoted by $\Omega_{\text{free}}\subseteq\Omega$. We assume that $\Omega_{\text{free}}$ is populated with $M>0$ static semantic objects. Each object $e$ is characterized by its location $\bbx_e$ and semantic label $c_e\in\ccalC$, where $\ccalC$ is a set collecting all semantic labels that the robot can recognize (e.g., `bottle' or `chair'). Notice that the occupied space $\Omega\setminus\Omega_{\text{free}}$ (e.g., walls) may prevent access to semantic objects of interest.
%
We assume that the robot is equipped with full knowledge of the environment allowing it to detect obstacles, classify, and navigate towards semantic objects. For example, the robots will know the location of the semantic objects and navigate to the objects' locations within obstacle-free space.

\subsection{Task Specification and Sequencing}

A team of $N$ robots is responsible for a high-level task $\phi$ comprised of $K$ sub-tasks expressed in natural language (NL). For example, such a high-level task is comprised of sub-tasks `deliver a can of Coke to location X; deliver a bottle of water to location Y', where in this case the number of sub-tasks is $2$. Notice that $\phi$ is expressed as a whole NL sentence such that we use existing LLMs to reason and determine which of the sub-tasks should be assigned to a specific robot. Each robot $i$ in the team will be assigned to a sequence of decisions generated by LLMs $\tau_i = s_i(0)\dots s_i(H)$ for some horizon $H\geq 1$. Due to the coordination requirement of multi-robot systems, robot ordering issues might also affect the outcome of the generated plan, we address this challenge in section III using a coordinate descent-based method. Here we assume the NL-based high-level task $\phi$ can be satisfied by a finite robot team trajectory $\tau$, defined as a finite sequence of decisions $s_i(t), i \in N$, i.e., $\tau=
\{ \tau_i(0) \}_{i=0}^N \dots \{ \tau_i(H-1) \}_{i=0}^N$. 
 
\subsection{Problem Statement}

This paper addresses the following problem:

\begin{problem}\label{pr:pr1}
    Given a team of $N$ homogeneous robots with known dynamics and capabilities, a known semantic environment $\Omega$, and an NL-based task $\phi$ comprise of several sub-tasks, design (online) a robot path $\tau_{\phi}$ satisfying $\phi$.
\end{problem}


\begin{ex}[Feasible Plan Example]
Consider a team of $3$ robots with skills $\ccalA=\{\text{go to}, \text{pick up}, \text{idle}\}$ residing in an environment shown in Fig. \ref{fig:env}. The semantic objects that each robot can recognize are $\ccalC=\{\text{Coke}, \text{Pen}, \text{Water Bottle}\}$. The environment along with the locations of all semantic objects is shown in Fig. \ref{fig:env}. 
%
The task of the robot is defined as: $\phi =$ `Deliver the Pen to location $\bbx_3$'; `Deliver a Coke to the desk at location $\bbx_3$'. A plan $\tau_{\phi}$ to satisfy $\phi$ is defined as $\tau=s_1(\text{go to}, \text{Pen},1),s_2(\text{go to}, \text{Coke},1), s_3(\text{idle},1),\\s_1(\text{pick up}, \text{Pen},2),s_2(\text{pick up}, \text{Coke},2), s_3(\text{idle},2),\\s_1(\text{go to}, \bbx_3,3),s_2(\text{go to}, \bbx_3,3), s_3(\text{idle},3)$. Notice that this plan has a horizon $H=3$ while robot $3$ remains idle all the time because all the sub-tasks can be satisfied using the remaining $2$ robots.
\label{ex:me} 
\end{ex}
